Improving KernelSHAP: Practical Shapley Value Estimation via Linear Regression

The Shapley value concept from cooperative game theory has become a popular technique for interpreting ML models, but efficiently estimating these values remains challenging, particularly in the model-agnostic setting. Here, we revisit the idea of estimating Shapley values via linear regression to understand and improve upon this approach. By analyzing the original KernelSHAP alongside a newly proposed unbiased version, we develop techniques to detect its convergence and calculate uncertainty estimates. We also find that the original version incurs a negligible increase in bias in exchange for significantly lower variance, and we propose a variance reduction technique that further accelerates the convergence of both estimators. Finally, we develop a version of KernelSHAP for stochastic cooperative games that yields fast new estimators for two global explanation methods.

==> Shapley Regression AISTATS 2021 (Camera Ready)/0_abstract.tex <==
\begin{abstract}%
    The Shapley value concept from cooperative game theory has become a popular technique for interpreting ML models, but efficiently estimating these values remains challenging, particularly in the model-agnostic setting. Here, we revisit the idea of estimating Shapley values via linear regression to understand and improve upon this approach. By analyzing the original KernelSHAP alongside a newly proposed unbiased version, we develop techniques to detect its convergence and calculate uncertainty estimates. We also find that the original version incurs a negligible increase in bias in exchange for significantly lower variance,
    % negligibly increases bias in exchange for significantly  reducing variance,
    and we propose a variance reduction technique that further accelerates the convergence of both estimators. Finally, we develop a version of KernelSHAP for stochastic cooperative games that yields fast new estimators for two global explanation methods.
\end{abstract}

==> Shapley Regression AISTATS 2021 (Camera Ready)/1_introduction.tex <==
\section{INTRODUCTION}

Shapley values are central to many machine learning (ML) model explanation methods (e.g., SHAP, IME, QII, Shapley Effects, Shapley Net Effects, SAGE) \cite{lundberg2017unified, lundberg2020local, vstrumbelj2014explaining, datta2016algorithmic, owen2014sobol, lipovetsky2001analysis, covert2020understanding}. Though developed in the cooperative game theory context \cite{shapley1953value}, recent work shows that Shapley values provide a powerful tool for explaining how models work when either individual features \cite{lundberg2017unified}, individual neurons in a neural network \cite{ghorbani2020neuron}, or individual samples in a dataset \cite{ghorbani2019data} are viewed as players in a cooperative game.
% Consequently, Shapley values have
% % it has
% become a go-to method for allocating credit and quantifying contributions in a principled manner.
They have become a go-to solution for allocating credit  and quantifying contributions due to to their appealing theoretical properties.
% when needing a principled way to allocate credit and predict feature contribution.
%\sandy{Since you just said that it has broader utility, I didn't want to end by referencing the cooperative game use specifically. Please clean up as you see fit.}

%in cooperative games.

The main challenge when using Shapley values is calculating them efficiently. A naive calculation has computational complexity that is exponential in the number of players, so numerous approaches have been proposed to accelerate their calculation.
% , sometimes using approximations.
Besides brute-force methods \cite{lipovetsky2001analysis}, other techniques include sampling-based approximations \cite{vstrumbelj2014explaining, song2016shapley, chen2018shapley, covert2020understanding}, model-specific approximations (e.g., TreeSHAP) \cite{ancona2019explaining, lundberg2020local} and a linear regression-based approximation (KernelSHAP) \cite{lundberg2017unified}.

Here, we revisit the regression-based approach to address several shortcomings in KernelSHAP. Recent work has questioned whether KernelSHAP is an unbiased estimator \cite{merrick2019explanation}, and, unlike sampling-based 
% Shapley value
estimators \cite{castro2009polynomial, maleki2013bounding, covert2020understanding}, KernelSHAP does not provide uncertainty estimates. Furthermore, it provides no guidance on the number of samples required because its convergence properties are not well understood.
% prior work has not closely examined its convergence properties.

We address each of these problems, in part by building on a newly proposed unbiased version of the regression-based approach. Our contributions include:

\begin{enumerate}
    \item Deriving an unbiased version of KernelSHAP and showing empirically that the original version incurs a negligible increase in bias in exchange for significantly lower variance
    % negligibly increases bias in exchange for significantly reducing the variance
    % \item
    % % By assuming that KernelSHAP's variance evolves at the same rate as the unbiased version, 
    % Showing how to detect
    % KernelSHAP's convergence, avoid specifying a number of samples, and calculate uncertainty estimates for the results
    \item Showing how to detect KernelSHAP's convergence, automatically determine the number of samples required, and calculate uncertainty estimates for the results
    \item Proposing a variance reduction technique that further accelerates KernelSHAP's convergence
    \item Adapting the regression-based approach
    % these estimators
    to stochastic cooperative games \cite{charnes1973prior} to provide fast new approximations for two global explanation methods, SAGE \cite{covert2020understanding} and Shapley Effects \cite{owen2014sobol}
\end{enumerate}

With these new insights and tools, we
% provide
offer a more practical approach to Shapley value estimation via linear regression.\footnote{\ttfamily \href{https://github.com/iancovert/shapley-regression}{https://github.com/iancovert/shapley-regression}}

==> Shapley Regression AISTATS 2021 (Camera Ready)/2_shapley.tex <==
\section{THE SHAPLEY VALUE}

We now provide background information on
% context for understanding
cooperative game theory and the Shapley value.

\subsection{Cooperative Games}

A \textit{cooperative game} is a function $v: 2^d \mapsto \R$ that returns a value for each coalition (subset) $S \subseteq D$, where $D = \{1, \ldots, d\}$ represents a set of \textit{players}. 
%\sandy{Commented following sentence out since it's repetitive.}
Cooperative game theory has become increasingly important in ML because many methods frame model explanation problems in terms of cooperative games \cite{covert2020explaining}.
Notably, SHAP~\cite{lundberg2017unified}, IME \cite{vstrumbelj2014explaining} and QII \cite{datta2016algorithmic} define cooperative games that represent an individual prediction's dependence on different features.
% prediction given a subset of features.
For a model $f$ and an input $x$, SHAP (when using the marginal distribution \cite{lundberg2017unified}) analyzes the cooperative game $v_x$, defined as

\begin{equation}
    v_x(S) = \E[f(x_S, X_{D \setminus S})],
\end{equation}

where $x_S \equiv \{x_i : i \in S\}$ represents a feature subset and $X_S$ is the corresponding random variable. Two other methods, Shapley Effects \cite{owen2014sobol} and SAGE \cite{covert2020understanding}, define cooperative games that represent a model's behavior across the entire dataset. For example, given a loss function $\ell$ and response variable $Y$, SAGE uses
% is based on
a cooperative game $w$ that represents the model's predictive performance given a subset of features $X_S$:

\begin{equation}
    w(S) = - \E\Big[\ell\big(\E[f(X) \; | \; X_S], Y\big)\Big]. \label{eq:sage_game}
\end{equation}

%\sandy{The following paragraph repeats information already in the Introduction and can be deleted IMO.}
Several other techniques also frame model explanation questions in terms of cooperative games, where
% each method observes how some
a target quantity (e.g., model loss) varies as groups of players (e.g., features) are removed, and the Shapley value summarizes each player's contribution \cite{covert2020explaining}.
% where players represent either individual features \cite{lipovetsky2001analysis}, neurons in a neural network \cite{ghorbani2020neuron}, or examples in a dataset \cite{ghorbani2019data}. Each technique observes how some target quantity (e.g., model loss) varies as groups of players (e.g., features) are removed, and the Shapley value summarizes each player's contribution.

\subsection{Shapley Values}

The Shapley value \cite{shapley1953value}
%is a celebrated cooperative game theory result for defining credit allocations to each player in a game \cite{shapley1953value}. It 
assumes that the \textit{grand coalition} $D$ is participating and seeks to provide each player with a fair allocation of the total profit, which is represented by $v(D)$. Fair allocations must be based on each player's contribution to the profit, but a player's contribution is often difficult to define. Player $i$'s \textit{marginal contribution} to the coalition $S$ is the difference $v(S \cup \{i\}) - v(S)$, but the marginal contribution typically depends on which players $S$ are already participating.

The Shapley value resolves this problem by deriving a unique value based on a set of fairness axioms; see \cite{shapley1953value, monderer2002variations} for further detail. It can be understood as a player's average marginal contribution across all possible player orderings, and each player's Shapley value $\phi_1(v), \ldots, \phi_d(v)$ for a game $v$ is given by:

\begin{equation}
    \phi_i(v) = \frac{1}{d} \sum_{S \subseteq D \setminus \{i\}} \binom{d - 1}{|S|}\inv \Big(v(S \cup \{i\}) - v(S)\Big). \label{eq:shapley}
\end{equation}

%\Sandy{Again, the following has already been stated.  I'd like to reduce repetition to get readers to the 'meat' of your proposal more efficiently.}
Many ML model explanation methods can be understood in terms of ideas from cooperative game theory \cite{covert2020explaining}, but the Shapley value is especially popular and is also widely used in other fields \cite{aumann1994economic, petrosjan2003time, tarashev2016risk}.

\subsection{Weighted Least Squares Characterization}

While we can characterize the  Shapley value in many ways, the perspective most relevant to our work is viewing it as a solution to a weighted least squares problem. Many works have considered fitting simple models to cooperative games \cite{charnes1988extremal, hammer1992approximations, grabisch2000equivalent, ding2008formulas, ding2010transforms, marichal2011weighted}, particularly additive models of the form

\begin{equation*}
    u(S) = \beta_0 + \sum_{i \in S} \beta_i.
\end{equation*}

Such additive models are known as \textit{inessential games}, and although a
% cooperative
game $v$ may not be inessential, an inessential approximation can help summarize
% provide a helpful summary of
each player's average contribution. Several works \cite{charnes1988extremal, hammer1992approximations, ding2008formulas} model games by solving a weighted least squares problem using a
weighting function $\mu$:

\begin{equation*}
    \min_{\beta_0, \ldots, \beta_d} \; \sum_{S \subseteq D} \mu(S) \Big(u(S) - v(S) \Big)^2.
\end{equation*}

Perhaps surprisingly, different weighting kernels $\mu$ lead to recognizable optimal regression coefficients $(\beta_1^*, \ldots \beta_d^*)$ \cite{covert2020explaining}. In particular, a carefully chosen weighting kernel yields optimal regression coefficients equal to the Shapley values \cite{charnes1988extremal, lundberg2017unified}. The Shapley kernel $\mu_{\mathrm{Sh}}$ is given by

\begin{equation*}
    \mu_{\mathrm{Sh}}(S) = \frac{d - 1}{\binom{d}{|S|}|S|(d - |S|)},
\end{equation*}

where the values $\mu_{\mathrm{Sh}}(\{\}) = \mu_{\mathrm{Sh}}(D) = \infty$ effectively enforce constraints $\beta_0 = v(\{\})$ for the intercept and $\sum_{i \in D} \beta_i = v(D) - v(\{\})$ for the sum of the coefficients. Lundberg and Lee \cite{lundberg2017unified} used this Shapley value interpretation when developing an approach to approximate SHAP values via linear regression.

==> Shapley Regression AISTATS 2021 (Camera Ready)/3_regression.tex <==
\section{LINEAR REGRESSION APPROXIMATIONS}

As noted, Shapley values are difficult to calculate because they require examining each player's marginal contribution to every possible subset (Eq.~\ref{eq:shapley}). This leads to run-times  that are exponential in the number of players, so efficient approximations are of great practical importance \cite{vstrumbelj2014explaining, song2016shapley, lundberg2017unified, chen2018shapley, ancona2019explaining, lundberg2020local, covert2020understanding}. Here, we revisit the regression-based approach presented by Lundberg and Lee (KernelSHAP) \cite{lundberg2017unified} and then present an unbiased version of this approach whose properties are simpler to analyze.
% that is simpler to analyze.

\subsection{Optimization Objective}

The least squares characterization of the Shapley value suggests that we can calculate the values $\phi_1(v), \ldots, \phi_d(v)$ by solving the optimization problem

\begin{align}
    &\min_{\beta_0, \ldots, \beta_d} \; \sum_{0 < |S| < d} \mu_{\mathrm{Sh}}(S) \Big(\beta_0 + \sum_{i \in S} \beta_i - v(S) \Big)^2 \nonumber \\
    &\mathrm{s.t.} \quad \beta_0 = v(\{\}), \quad \beta_0 + \sum_{i = 1}^d \beta_i = v(D). \label{eq:constrained_problem}
\end{align}

\textbf{Notation.} We introduce new notation to make the problem easier to solve. First, we denote the non-intercept coefficients as $\beta = (\beta_1, \ldots, \beta_d) \in \R^d$. Next, we denote each subset $S \subseteq D$ using the corresponding binary vector $z \in \{0, 1\}^d$, and with tolerable abuse of notation we write $v(z) \equiv v(S)$ and $\mu_{\mathrm{Sh}}(z) \equiv \mu_{\mathrm{Sh}}(S)$ for $S = \{i : z_i = 1\}$. Lastly, we denote a distribution over $Z$ using $p(z)$, where we define $p(z) \propto \mu_{\mathrm{Sh}}(z)$ when $0 < \mathbf{1}^Tz < d$ and $p(z) = 0$ otherwise. With this, we can
% now
rewrite the optimization problem as 

% \begin{align}
%     &\min_{\beta_0, \ldots, \beta_d} \; \sum_z p(z) \Big(\beta_0 + z^T \beta - v(z) \Big)^2 \nonumber \\
%     &\mathrm{s.t.} \quad \beta_0 = v(\mathbf{0}), \quad \mathbf{1}^T \beta = v(\mathbf{1}) - v(\mathbf{0}). \label{eq:problem}
% \end{align}
\begin{align}
    &\min_{\beta_0, \ldots, \beta_d} \; \sum_z p(z) \Big(v(\mathbf{0}) + z^T \beta - v(z) \Big)^2 \nonumber \\
    &\mathrm{s.t.}
    % \quad \beta_0 = v(\mathbf{0}),
    \quad\quad \mathbf{1}^T \beta = v(\mathbf{1}) - v(\mathbf{0}). \label{eq:problem}
\end{align}

\subsection{Dataset Sampling} \label{sec:sampling}

Solving the problem in Eq.~\ref{eq:problem} requires evaluating the cooperative game $v$ with all $2^d$ coalitions. Evaluating $v(\mathbf{0})$ and $v(\mathbf{1})$ is sufficient to ensure that the constraints are satisfied, but all values $v(z)$ for $z$ such that $0 < \mathbf{1}^Tz < d$ are required to fit the model exactly. KernelSHAP manages this challenge by subsampling a dataset and optimizing an approximate objective. We refer to this approach as \textit{dataset sampling}.
% \textit{approximate objective}.
Using $n$ independent samples $z_i \sim p(Z)$ and their values $v(z_i)$, KernelSHAP solves the following
% approximate
% version of the
problem:

% \begin{align}
%     &\min_{\beta_0, \ldots, \beta_d} \; \frac{1}{n} \sum_{i = 1}^n \Big(\beta_0 + z_i^T \beta - v(z_i) \Big)^2 \nonumber \\
%     &\mathrm{s.t.} \quad \beta_0 = v(\mathbf{0}), \quad \mathbf{1}^T \beta = v(\mathbf{1}) - v(\mathbf{0}). \label{eq:approximate_problem}
% \end{align}
\begin{align}
    &\min_{\beta_0, \ldots, \beta_d} \; \frac{1}{n} \sum_{i = 1}^n \Big(v(\mathbf{0}) + z_i^T \beta - v(z_i) \Big)^2 \nonumber \\
    &\mathrm{s.t.}
    % \quad \beta_0 = v(\mathbf{0}),
    \quad\quad \mathbf{1}^T \beta = v(\mathbf{1}) - v(\mathbf{0}). \label{eq:approximate_problem}
\end{align}

% A similar
The dataset sampling approach, also applied by LIME \cite{ribeiro2016should}, offers the flexibility to use only enough samples
% the number of samples required
to accurately approximate the objective. Given a set of samples $(z_1, \ldots, z_n)$, solving this problem is straightforward. The Lagrangian with multiplier $\nu \in \R$ is given by:

\begin{align*}
    \hat{\mathcal{L}}(\beta, \nu) = \; &\beta^T \Big(\frac{1}{n} \sum_{i = 1}^n z_iz_i^T\Big) \beta \nonumber \\
    &- 2 \beta^T \Big( \frac{1}{n} \sum_{i = 1}^n z_i \big(v(z_i) - v(\mathbf{0})\big) \Big) \nonumber \\
    &+ \frac{1}{n} \sum_{i = 1}^n \big(v(z_i) - v(\mathbf{0})\big)^2 \nonumber \\
    &+ 2\nu \big(\mathbf{1}^T \beta - v(\mathbf{1}) + v(\mathbf{0})\big).
\end{align*}

If we introduce the shorthand notation

\begin{align*}
    \hat A_n = \frac{1}{n} \sum_{i = 1}^n z_iz_i^T \quad\mathrm{and}\quad
    \hat b_n = \frac{1}{n} \sum_{i = 1}^n z_i \Big(v(z_i) - v(\mathbf{0})\Big),
\end{align*}

then we can use the problem's KKT conditions \cite{boyd2004convex} to derive the following solution:

\begin{align}
    \hat{\beta}_n &= \hat A_n\inv \Big(\hat b_n - \mathbf{1} \frac{\mathbf{1}^T \hat A_n\inv \hat b_n - v(\mathbf{1}) + v(\mathbf{0})}{\mathbf{1}^T \hat A_n\inv \mathbf{1}}\Big). \label{eq:sampled_solution}
\end{align}

This method is known as KernelSHAP \cite{lundberg2017unified}, and the implementation in the SHAP repository\footnote{\url{http://github.com/slundberg/shap}} also allows for regularization terms in the approximate objective (Eq.~\ref{eq:approximate_problem}), such as the $\ell_1$ penalty \cite{tibshirani1996regression}. While this approach is intuitive and simple to implement, the estimator $\hat{\beta}_n$ is surprisingly difficult to characterize. As we show in Section~\ref{sec:estimator_properties}, it is unclear whether it is unbiased, and understanding its variance and rate of convergence is not straightforward. Therefore, we derive an alternative approach that is simpler to analyze.

\subsection{An Exact Estimator} \label{sec:exact}

Consider the solution to the problem that uses all $2^d$ player coalitions (Eq.~\ref{eq:problem}). Rather than finding an \textit{exact solution to an approximate problem} (Section~\ref{sec:sampling}), we now derive an \textit{approximate solution to the exact problem}. The full problem's Lagrangian is given by

\begin{align*}
    \mathcal{L}(\beta, \nu) = \; &\beta^T \E[ZZ^T] \beta \nonumber \\
    &- 2 \beta^T \E\Big[Z \big(v(Z) - v(\mathbf{0})\big) \Big] \nonumber \\
    &+ \E\Big[\big(v(Z) - v(\mathbf{0})\big)^2\Big] \nonumber \\
    &+ 2\nu \big(\mathbf{1}^T \beta - v(\mathbf{1}) + v(\mathbf{0})\big),
\end{align*}

where we now consider $Z$ to be a random variable distributed according to $p(Z)$. Using the shorthand notation

\begin{align*}
    A = \E[ZZ^T] \quad\mathrm{and}\quad b = \E\Big[Z \big(v(Z) - v(\mathbf{0})\big)\Big],
\end{align*}

we can write the solution to the exact problem as:

\begin{equation}
    \beta^* = A\inv \Big(b - \mathbf{1} \frac{\mathbf{1}^T A\inv b - v(\mathbf{1}) + v(\mathbf{0})}{\mathbf{1}^T A\inv \mathbf{1}}\Big). \label{eq:solution}
\end{equation}

Due to our setup of the optimization problem, we have the property that $\beta_i^* = \phi_i(v)$. Unfortunately, we cannot evaluate this expression in practice without evaluating $v$ for all $2^d$ coalitions $S \subseteq D$.

However, knowledge of $p(Z)$ means that $A \in \R^{d \times d}$ can be calculated exactly and efficiently. To see this, note that $(ZZ^T)_{ij} = Z_iZ_j = \mathbbm{1}(Z_i = Z_j = 1)$. Therefore, to calculate $A$, we need to estimate only  $p(Z_i = 1)$ for diagonal values $A_{ii}$ and $p(Z_i = Z_j = 1)$ for off-diagonal values $A_{ij}$. See Appendix~\ref{app:exact} for their derivations.

Since $b$ cannot be calculated exactly and efficiently due to its dependence on $v$, this suggests that we should use $A$'s exact form and approximate $\beta^*$ by estimating (only) $b$. We propose the following estimator for $b$:
% as an estimator for $b$:

\begin{equation*}
    \bar b_n = \frac{1}{n} \sum_{i = 1}^n z_i v(z_i) - \E[Z] v(\mathbf{0}).
\end{equation*}

Using this, we arrive at an
% the following
alternative to the original KernelSHAP estimator, which we refer to as \textit{unbiased KernelSHAP}:

\begin{align}
    \bar{\beta}_n = A\inv \Big(\bar b_n - \mathbf{1} \frac{\mathbf{1}^T A\inv \bar b_n - v(\mathbf{1}) + v(\mathbf{0})}{\mathbf{1}^T A\inv \mathbf{1}}\Big). \label{eq:modified_solution}
\end{align}

In the next section, we compare these two approaches both theoretically and empirically.


==> Shapley Regression AISTATS 2021 (Camera Ready)/4_properties.tex <==
\section{ESTIMATOR PROPERTIES} \label{sec:estimator_properties}

We now analyze the consistency, bias and variance properties of the Shapley value estimators, and we consider how to detect, forecast, and accelerate their convergence.

\subsection{Consistency, Bias and Variance} \label{sec:properties}

A \textit{consistent} estimator is one that converges to the correct Shapley values $\beta^*$ given a sufficiently large number of samples. If the game $v$ has bounded value, then the strong law of large numbers implies that

\begin{equation*}
    \lim_{n \to \infty} \hat A_n = A \quad\mathrm{and}\quad \lim_{n \to \infty} \hat b_n = \lim_{n \to \infty} \bar b_n = b,
\end{equation*}

where the convergence is almost sure. From this, we see that both estimators are consistent:

\begin{equation*}
    \lim_{n \to \infty} \; \hat{\beta}_n = \lim_{n \to \infty} \; \bar{\beta}_n = \beta^*.
\end{equation*}

Next, an \textit{unbiased} estimator is one whose expectation is equal to the correct Shapley values $\beta^*$. This is difficult to verify for the KernelSHAP estimator $\hat{\beta}_n$ due to the interaction between $\hat A_n$ and $\hat b_n$ (see Eq.~\ref{eq:sampled_solution}). Both $\hat A_n$ and $\hat b_n$ are unbiased, but terms such as $\E[\hat A_n\inv \hat b_n]$ and $\E[\hat A_n\inv \mathbf{1} \mathbf{1}^T \hat A_n\inv \hat b_n / (\mathbf{1}^T \hat A_n\inv \mathbf{1})]$ are difficult to characterize. To make any claims about KernelSHAP's bias, we rely instead on empirical observations.

In contrast, it is easy to see that the alternative estimator $\bar \beta_n$ is unbiased. Because of its linear dependence on $\bar b_n$ and the fact that $\E[\bar b_n] = b$, we can see that

\begin{equation*}
    \E[\bar{\beta}_n] = \beta^*.
\end{equation*}

We therefore conclude that the alternative estimator $\bar{\beta}_n$ is both consistent and unbiased, whereas the original KernelSHAP ($\hat{\beta}_n$) is only provably consistent. It is for this reason that we refer to
% In the remainder of this work, we refer to
$\bar \beta_n$ as \textit{unbiased KernelSHAP}.

Regarding the estimators' variance, unbiased KernelSHAP is once again simpler to characterize. The values $\bar \beta_n$ are a function of $\bar b_n$, and the multivariate central limit theorem (CLT)  \cite{van2000asymptotic} asserts that $\bar b_n$ converges in distribution to a multivariate Gaussian, or

\begin{equation}
    \bar b_n \sqrt{n} \xrightarrow{D} \mathcal{N}(b, \Sigma_{\bar b}) \label{eq:clt},
\end{equation}

where $\Sigma_{\bar b} = \Cov\big(Zv(Z)\big)$. This implies that for the estimator $\bar \beta_n$, we have the convergence property

\begin{equation}
    \bar{\beta}_n \sqrt{n} \xrightarrow{D} \mathcal{N}(\beta^*, \Sigma_{\bar \beta}),
\end{equation}

where, due to its linear dependence on $\bar b_n$ (see Eq.~\ref{eq:modified_solution}), we have the covariance $\Sigma_{\bar \beta}$ given by

\begin{align}
    \Sigma_{\bar \beta} &= C \Sigma_{\bar b} C^T \\
    C &= A\inv - \frac{A\inv \mathbf{1} \mathbf{1}^T A\inv}{\mathbf{1}^T A\inv \mathbf{1}}. \label{eq:C}
\end{align}

This allows us to reason about unbiased KernelSHAP's asymptotic distribution. In particular, we remark that $\bar \beta_n$ has variance that reduces at a rate of $\mathcal{O}(\frac{1}{n})$.

In comparison, the original KernelSHAP estimator $\hat{\beta}_n$ is difficult to analyze due to the interaction between the $\hat A_n$ and $\hat b_n$ terms. We can apply the 
%\sandy{Spell out CLT first, or will readers already know the acronym?}
CLT to either term individually, but reasoning about $\hat{\beta}_n$'s distribution or variance remains challenging.

To facilitate our analysis of KernelSHAP, we present a simple experiment to compare the two estimators. We approximated the SHAP values for an individual prediction in the census income dataset \cite{lichman2013uci} and empirically calculated the mean squared error relative to the true SHAP values\footnote{The true SHAP values use a sufficient number of samples to ensure convergence (see Section~\ref{sec:convergence}).} across 250 runs. We then decomposed the error into bias and variance terms as follows:

\begin{equation*}
    \underbrace{\E\big[||\hat \beta_n - \beta^*||^2\big]}_{\text{Error}} = \underbrace{\E\big[||\hat \beta_n - \E[\hat \beta_n]||^2\big]}_{\text{Variance}} + \underbrace{\big|\big|\E[\hat \beta_n] - \beta^*\big|\big|^2.}_{\text{Bias}}
\end{equation*}

Figure~\ref{fig:error} shows that the error for both estimators is dominated by variance rather than bias.\footnote{The unbiased approach appears to have higher bias due to estimation error, but its bias is provably zero.} It also shows that KernelSHAP incurs virtually no bias in exchange for significantly lower variance. In Appendix~\ref{app:convergence_experiments}, we provide global measures of the bias and variance to confirm these observations across multiple examples and two other datasets. This suggests that although KernelSHAP is more difficult to analyze theoretically, it should be used in practice because its bias is negligible
% (yet not provably zero)
and it converges faster.

\input{inserts/error}

\subsection{Variance Reduction via Paired Sampling} \label{sec:var_reduction}

Having
% Once we have
analyzed each estimator's properties, we now consider whether their convergence can be accelerated. We propose a simple variance reduction technique that leads to significantly faster convergence in practice.

When sampling $n$ subsets according to the distribution $z_i \sim p(Z)$, we suggest a \textit{paired sampling} strategy where each sample $z_i$ is paired with its complement\footnote{We call $\mathbf{1} - z$ the \textit{complement} because it is the binary vector for $D \setminus S$, where $S$ corresponds to $z$.} $\mathbf{1} - z_i$. To show why this approach accelerates convergence, we focus on unbiased KernelSHAP, which is easier to analyze theoretically.

When estimating $b$ for unbiased KernelSHAP ($\bar \beta_n$), consider using the following modified estimator that combines $z_i$ with $\mathbf{1} - z_i$:

\vskip - 0.1in

\begin{equation}
    \check b_{n} = \frac{1}{2n} \sum_{i = 1}^n \big( z_i v(z_i) + (\mathbf{1} {-} z_i) v(\mathbf{1} {-} z_i) - v(\mathbf{0}) \big).
\end{equation}

Substituting this into unbiased KernelSHAP (Eq.~\ref{eq:modified_solution}) yields a new estimator $\check{\beta}_n$ that preserves the properties of being both consistent and unbiased:

\vskip - 0.1in

\begin{equation}
    \check{\beta}_{n} = A\inv \Big(\check b_{n} - \mathbf{1} \frac{\mathbf{1}^T A\inv \check b_{n} - v(\mathbf{1}) + v(\mathbf{0})}{\mathbf{1}^T A\inv \mathbf{1}}\Big). \label{eq:reduced_solution}
\end{equation}

For games $v$ that satisfy a specific condition, we can guarantee that this sampling approach leads to $\check \beta_n$ having lower variance than $\bar \beta_n$, even when we account for $\check b_n$ requiring twice as many cooperative game evaluations as $\bar b_n$ (see proof in Appendix~\ref{app:variance_reduction}).

\vskip 0.1in

\begin{theorem} \label{thm:confidence}
    The difference between the covariance matrices for the estimators $\bar \beta_{2n}$ and $\check \beta_n$ is given by
    
    \vskip - 0.05in
    
    \begin{equation*}
        \Cov(\bar \beta_{2n}) - \Cov(\check \beta_n) = \frac{1}{2n} C G_v C^T,
    \end{equation*}
    
    \vskip - 0.05in
    
    where $G_v$ is a property of the game $v$, defined as
    
    \vskip - 0.05in
    
    \begin{equation*}
        G_v = - \Cov\Big(Zv(Z), (\mathbf{1} - Z) v(\mathbf{1} - Z)\Big).
    \end{equation*}
    
    \vskip - 0.05in
    
    For sufficiently large $n$, $G_v \succeq 0$ guarantees that the Gaussian confidence ellipsoid $\bar E_{2n, \alpha}$ for $\bar \beta_{2n}$ contains the corresponding confidence ellipsoid $\check E_{n, \alpha}$ for $\check \beta_{n}$, or $\check E_{n, \alpha} \subseteq \bar E_{2n, \alpha}$,
    at any confidence level $\alpha \in (0, 1)$.
\end{theorem}

Theorem~\ref{thm:confidence} shows that $\check \beta_n$ is a more precise estimator than $\bar \beta_{2n}$ when the condition $G_v \succeq 0$ is satisfied (i.e., $G_v$ is positive semi-definite). This may not hold in the general case, but in Appendix~\ref{app:variance_reduction} we show that a weaker condition holds for \textit{all games}: the diagonal values of $G_v$ satisfy $(G_v)_{ii} \geq 0$ for any game $v$. Geometrically, this weaker condition means that $\bar E_{2n, \alpha}$ extends beyond $\check E_{n, \alpha}$ in the axis-aligned directions.

\input{inserts/confidence}

Figure~\ref{fig:confidence} illustrates the result of Theorem~\ref{thm:confidence} by showing empirical 95\% confidence ellipsoids for two SHAP values. Although a comparable condition is difficult to derive for the original KernelSHAP estimator ($\hat \beta_n$), we find that the paired sampling approach yields a similar reduction in variance. Our experiments provide further evidence that this approach accelerates convergence for both estimators (Section~\ref{sec:experiments}).

\subsection{Convergence Detection and Forecasting} \label{sec:convergence}

One of KernelSHAP's practical shortcomings is its lack of guidance on the number of samples required to obtain accurate estimates. We address this problem by developing an approach for convergence detection and forecasting.

Previously, we showed that unbiased KernelSHAP ($\bar \beta_n$) has variance that reduces at a rate $\mathcal{O}(\frac{1}{n})$ (Eq.~\ref{eq:clt}). Furthermore, its variance is simple to estimate in practice: we require only an empirical estimate $\hat \Sigma_{\bar b}$ of $\Sigma_{\bar b}$ (defined above), which we can calculate using an online algorithm, such as Welford's \cite{welford1962note}.

We also showed that the original KernelSHAP ($\hat \beta_n$) is difficult to characterize, but its variance is empirically lower than the unbiased version. Understanding its variance is useful for convergence detection, so we propose an approach for approximating it. Based on the results in Figure~\ref{fig:error}, we may hypothesize that KernelSHAP's variance reduces at the same rate of $\mathcal{O}(\frac{1}{n})$; in Appendix~\ref{app:convergence_experiments}, we examine this by plotting the product of the variance and the number of samples over the course of estimation. We find that the product is \textit{constant} as the sample number increases, which suggests that the $\mathcal{O}(\frac{1}{n})$ rate holds in practice. This property is difficult to prove formally, but it can be used for simple variance approximation.
% we verify that this holds across multiple examples and several datasets. Although this property is difficult to prove formally, it holds in practice and permits a simple variance approximation.

When running KernelSHAP, we suggest estimating the variance by selecting an intermediate value $m$ such that $m << n$ and calculating multiple independent estimates $\hat \beta_m$ while accumulating samples for $\hat \beta_n$. For any $n$, we can then approximate $\Cov(\hat \beta_n)$ as

\begin{equation*}
    \Cov(\hat \beta_n) \approx \frac{m}{n}\Cov(\hat \beta_m),
\end{equation*}

where $\Cov(\hat \beta_m)$ is estimated empirically using the multiple independent estimates $\hat \beta_m$. This online approach has a negligible impact on the algorithm's run-time, and the covariance estimate can be used to provide confidence intervals for the final results.

Whether we use the original or unbiased version of KernelSHAP, the estimator's covariance at a given value of $n$ lets us both detect and forecast convergence. For detection, we propose stopping at the current value $n$ when the largest standard deviation is a sufficiently small portion $t$ (e.g., $t = 0.01$) of the gap between the largest and smallest Shapley value estimates. For unbiased KernelSHAP, this criterion is equivalent to:

\begin{equation*}
    \max_i \sqrt{\frac{1}{n}(\hat \Sigma_{\bar \beta})_{ii}} < t \Big( \max_i \; (\bar{\beta}_n)_i - \min_i \; (\bar{\beta}_n)_i \Big).
\end{equation*}

To forecast the number of samples required to reach convergence, we again invoke
% also use
the property that estimates have variance that reduces at a rate of $\mathcal{O}(\frac{1}{n})$. Given a value $t$ and estimates $\bar{\beta}_n$ and $\hat \Sigma_{\bar \beta}$, the approximate number of samples $\hat N$ required is:

\begin{equation*}
    \hat N = \frac{1}{t^2} \Big(\frac{\max_i \; \sqrt{(\hat \Sigma_{\bar \beta})_{ii}}}{\max_i \; (\bar{\beta}_n)_i - \min_i \; (\bar{\beta}_n)_i}\Big)^2. \label{eq:forecast}
\end{equation*}

This allows us to forecast the time until convergence at any point during the algorithm. The forecast is expected to become more accurate as the estimated terms become more precise.

Our approach is theoretically grounded for unbiased KernelSHAP, and the approximate approach for the standard version of KernelSHAP relies only on the assumption that $\Cov(\hat \beta_n)$ reduces at a rate of $\mathcal{O}(\frac{1}{n})$. Appendix~\ref{app:algorithms} shows algorithms for both approaches, which illustrate both variance reduction and convergence detection techniques.

==> Shapley Regression AISTATS 2021 (Camera Ready)/5_stochastic.tex <==
\input{inserts/examples}

\section{STOCHASTIC COOPERATIVE GAMES}

We have thus far focused on developing a regression-based approach to estimate Shapley values for any cooperative game. We now discuss how to adapt this approach to stochastic cooperative games, which leads to fast estimators for two global explanation methods.

\subsection{Stochastic Cooperative Games}

\textit{Stochastic cooperative games} return a random value for each coalition of participating players $S \subseteq D$. Such games are represented by a function $V$ that maps coalitions to a \textit{distribution} of possible outcomes, so that $V(S)$ is a random variable \cite{charnes1973prior, charnes1976coalitional}. 

To aid our presentation, we assume that the uncertainty in the game can be represented by an exogenous random variable $U$. The game can then be denoted by $V(S, U)$, where $V(\cdot, U)$ is a deterministic function of $S$ for any fixed value of the variable $U$.

Stochastic cooperative games provide a useful tool for understanding two global explanation methods, SAGE \cite{covert2020understanding} and Shapley Effects \cite{owen2014sobol}. To see why, assume an exogenous variable $U = (X, Y)$ that represents a random input-label pair, and consider the following game:

\begin{equation}
    W(S, X, Y) = - \ell\Big(\E\big[f(X) | X_S\big], Y\Big).
    % W(S, x, y) = - \ell\Big(\E\big[f(X) | X_S = x_S\big], y\Big).
\end{equation}

The game $W$ evaluates the (negated) loss with respect to the label $Y$ given a prediction that depends only on the features $X_S$. The cooperative game used by SAGE can be understood as the expectation of this game, or $w(S) = \E_{XY}\big[W(S, X, Y)\big]$ (see Eq.~\ref{eq:sage_game}). Shapley Effects is based on the expectation of a similar game, where the loss is evaluated with respect to the full model prediction $f(X)$ (see Appendix~\ref{app:shapley_effects}). As we show next, an approximation approach tailored to this setting yields significantly faster estimators for these methods.

\subsection{Generalizing the Shapley Value} \label{sec:generalizing}

It is natural to assign values to players in stochastic cooperative games like we do for deterministic games. We propose a simple generalization of the Shapley value for games $V(S, U)$ that averages a player's marginal contributions over both (i) player orderings and (ii) values of the exogenous variable $U$:

\begin{equation*}
    \phi_i(V) = \frac{1}{d} {\sum_{S {\subseteq} D {\setminus} \{i\}}} \binom{d {-} 1}{|S|}^{{-}1} \E_U \Big[ V(S \cup \{i\}, U) {-} V(S, U) \Big]. \label{eq:stochastic_shapley}
\end{equation*}

Due to the linearity property of Shapley values \cite{shapley1953value, monderer2002variations}, the following sets of values are equivalent:

\begin{enumerate}
    \item The Shapley values of the game's expectation $\bar v(S) = \E_U[V(S, U)]$, or $\phi_i(\bar v)$
    \item The expected Shapley values of games with fixed $U$, or $\E_U[\phi_i(v_U)]$ where $v_u(S) = V(S, u)$
    \item Our generalization of Shapley values to the stochastic cooperative game $V(S, U)$, or $\phi_i(V)$
\end{enumerate}

The first two list items suggest ways of calculating the values $\phi_i(V)$ using tools designed for deterministic cooperative games. However, the expectation $\E_U\big[V(S, U)\big]$ may be slow to evaluate (e.g., if it is across an entire dataset), and calculating Shapley values separately for each value of $U$ would be intractable if $U$ has many possible values. We therefore introduce a third approach.

\subsection{Shapley Value Approximation for Stochastic Cooperative Games} \label{sec:stochastic_kernelshap}

We now propose a fast, regression-based approach for calculating the generalized Shapley values $\phi_i(V)$ of stochastic cooperative games $V(S, U)$. Fortunately, it requires only a simple modification of the preceding approaches.

\input{inserts/forecasting}

First, we must calculate the values $\E_U\big[ V(\mathbf{1}, U) \big]$ and $\E_U \big[ V(\mathbf{0}, U) \big]$ for the grand coalition and the empty coalition. Next, we replace our previous $b$ estimators ($\hat b_n$ and $\bar b_n$) with estimators that use $n$ pairs of independent samples $z_i \sim p(Z)$ and $u_i \sim p(U)$. To adapt the original KernelSHAP to this setting, we use

\begin{equation*}
    \tilde b_n = \frac{1}{2} \sum_{i = 1}^n z_i \big(  V(z_i, u_i) - \E_U\big[V(\mathbf{0}, U)\big] \big).
\end{equation*}

We then substitute this into the KernelSHAP estimator, as follows:

\begin{equation}
    \tilde \beta_n = \hat A_n\inv \Big(\tilde b_{n} - \mathbf{1} \frac{\mathbf{1}^T \hat A_n\inv \tilde b_{n} - v(\mathbf{1}) + v(\mathbf{0})}{\mathbf{1}^T \hat A_n\inv \mathbf{1}}\Big). \label{eq:stochastic_solution}
\end{equation}

By the same argument used in Section~\ref{sec:sampling}, this approach estimates a solution to the weighted least squares problem whose optimal solution is the generalized Shapley values $\phi_i(V)$. This adaptation of KernelSHAP is consistent, and the analogous version of unbiased KernelSHAP is consistent and unbiased (see Appendix~\ref{app:stochastic}). These can be run with our paired sampling approach, and we can also provide uncertainty estimates and detect convergence (Section~\ref{sec:estimator_properties}).

==> Shapley Regression AISTATS 2021 (Camera Ready)/6_experiments.tex <==
\section{EXPERIMENTS} \label{sec:experiments}

We conducted experiments with four datasets to demonstrate the advantages of our Shapley value estimation approach. We used the census income dataset \cite{lichman2013uci}, the Portuguese bank marketing dataset \cite{moro2014data}, the German credit dataset \cite{lichman2013uci}, and a breast cancer (BRCA) subtype classification dataset \cite{berger2018comprehensive}. To avoid overfitting with the BRCA data, we analyzed a random subset of 100 out of 17,814 genes (Appendix~\ref{app:experiments}). We trained a LightGBM model \cite{ke2017lightgbm} for the census data, CatBoost \cite{prokhorenkova2018catboost} for the credit and bank data, and logistic regression for the BRCA data. Code for our experiments is available online.
% \footnote{\ttfamily \href{https://github.com/iancovert/shapley-regression}{http://github.com/iancovert/shapley-regression}}

\input{inserts/acceleration}

\input{inserts/shap_comparison}

To demonstrate local and global explanations with uncertainty estimates, we show examples of SHAP \cite{lundberg2017unified} and SAGE \cite{covert2020understanding} values generated using our estimators (Figure~\ref{fig:examples}). Both explanations used a convergence threshold of $t = 0.01$ and display 95\% confidence intervals, \textbf{which are features not previously offered by KernelSHAP}. We used the dataset sampling approach for both explanations, and for SAGE we used the estimator designed for stochastic cooperative games.
% ($\tilde \beta_n$).
These estimators are faster than their unbiased versions, but the results are nearly identical.

To measure run-time differences between each estimator when calculating SHAP values, we compared the number of samples required to explain 100 instances for each dataset (Table~\ref{tab:shap_comparison}). Rather than reporting the exact number of samples, which is dependent on the convergence threshold, we show the \textit{ratio} between the number of samples required by each estimator; this ratio is independent of the convergence threshold when convergence is defined by the mean squared estimation error falling below a fixed value (Appendix~\ref{app:experiments}). Table~\ref{tab:shap_comparison} displays results based on 100 runs for each instance. Results show that the dataset sampling approach (original) is consistently faster than the unbiased estimator, and that paired sampling enables significantly faster convergence. In particular, we find that our paired sampling approach yields a \textbf{$\mathbf{9\times}$ speedup on average over the original KernelSHAP.}

To investigate the accuracy of our convergence forecasting method, we compared the predicted number of samples to the true number across 250 runs. The number of samples depends on the convergence threshold, and we used a threshold $t = 0.005$ for SHAP and $t = 0.02$ for Shapley Effects and SAGE. Figure~\ref{fig:forecasting} shows the results for SHAP (using the census data), Shapley Effects (using the bank data) and SAGE (using the BRCA data). In all three cases, \textbf{the forecasts become more accurate with more samples, and they vary within an increasingly narrow range around the true number of required samples.} There is a positive bias in the forecast, but the bias diminishes with more samples.
%\sandy{I wanted the reader to be able to get the take-aways by having them stand out from rest of the text. Please check that I've bolded the correct highlights below.}

Finally, to demonstrate the speedup from our approach for stochastic cooperative games, we show that our stochastic estimator converges faster than a naive estimator based on the underlying game's expectation (see Section~\ref{sec:generalizing}). We plotted the ratio between the maximum standard deviation and the gap between the smallest and largest values, which we used to detect convergence (using a threshold $t = 0.01$).  Figure~\ref{fig:acceleration} shows that the stochastic approach dramatically speeds up both SAGE (using the BRCA data) and Shapley Effects (using the bank data), and that the paired sampling technique accelerates convergence for all estimators. The estimators based on the game's expectation are prohibitively slow and could not be run to convergence. \textbf{The fastest estimators for both datasets are stochastic estimators using the paired sampling technique,} and only these methods converged for both datasets in the number of samples displayed. As is the case for SHAP, the dataset sampling approach is often faster than the unbiased approach, but the latter is slightly faster for SAGE when using paired sampling.


==> Shapley Regression AISTATS 2021 (Camera Ready)/7_conclusion.tex <==
\section{DISCUSSION}

This paper described several approaches for estimating Shapley values via linear regression. We first introduced an unbiased version of KernelSHAP, with  properties that are simpler to analyze than the original version. We then developed techniques for detecting convergence, calculating uncertainty estimates, and reducing the variance of both the original and unbiased estimators. Finally, we adapted our approach to provide significantly faster estimators for two global explanation methods based on stochastic cooperative games. Our work makes significant strides towards improving the practicality of Shapley value estimation by automatically determining the required number of samples, providing confidence intervals, and accelerating the estimation process.

More broadly, our work contributes to a mature literature on Shapley value estimation \cite{castro2009polynomial, maleki2013bounding} and to the growing ML model explanation field \cite{owen2014sobol, vstrumbelj2014explaining, datta2016algorithmic, lundberg2017unified, covert2020understanding}. We  focused on improving the regression-based approach to Shapley value estimation, and we leave to future work a detailed comparison of this approach to sampling-based \cite{vstrumbelj2014explaining, song2016shapley, chen2018shapley, covert2020understanding} and model-specific approximations \cite{ancona2019explaining, lundberg2020local}. We also believe that certain insights from our work may be applicable to LIME, which is based on a similar dataset sampling approach; recent work has noted LIME's high variance when using an insufficient number of samples \cite{bansal2020sam}, and an improved understanding of its convergence properties
% its convergence properties have been the subject of recent research
\cite{garreau2020looking, mardaoui2020analysis} may lead to approaches for automatic convergence detection and uncertainty estimation.

% Prior work has noted LIME's high variance when using an insufficient number of samples \cite{bansal2020sam}, and recent work has developed concentration results to analyze LIME's convergence properties \cite{garreau2020looking, mardaoui2020analysis}. For future work, a
%\sandy{Below, what do you mean by "a similar" approach?  "Our approach"? If latter, which aspect?}
% similar approach may prove useful for developing a convergence detection and forecasting method for LIME.

==> Shapley Regression AISTATS 2021 (Camera Ready)/algorithms/kernelshap.tex <==
\begin{algorithm}[t]
\SetAlgoLined
\DontPrintSemicolon
\KwIn{Game $v$, convergence threshold $t$, intermediate samples $m$}
\tcp{Initialize}
n = 0\;
A = 0\;
b = 0\;
{}\;
\tcp{For tracking intermediate samples}
counter = 0\;
Atemp = 0\;
btemp = 0\;
estimates = list() \;
{}\;
\tcp{Sampling loop}
converged = False\;
\While{\upshape not converged}{
    \tcp{Draw next sample}
    Sample $z \sim p(Z)$\;
    \uIf{\upshape variance reduction}{
        Asample = $\frac{1}{2} \big( zz^T + (\mathbf{1} - z)(\mathbf{1} - z)^T \big)$\;
        bsample = $\frac{1}{2} \big(zv(z) + (\mathbf{1} {-} z)v(\mathbf{1} {-} z) - v(\mathbf{0})\big)$\;
    }
    \uElse{
        Asample = $zz^T$\;
        bsample = $z \big( v(z) - v(\mathbf{0})\big)$\;
    }
    {}\;
    \tcp{Welford's algorithm}
    n = n + 1\;
    A += (Asample $-$ A) / n \;
    b += (bsample $-$ b) / n\;
    counter += 1\;
    Atemp += (Asample $-$ Atemp) / counter \;
    btemp += (bsample $-$ btemp) / counter\;
    {}\;
    \uIf{\upshape counter == $m$}{
        \tcp{Get intermediate estimate}
        $\beta_m = \mathrm{Atemp}\inv \Big(\mathrm{btemp} - \mathbf{1} \frac{\mathbf{1}^T \mathrm{Atemp}\inv \mathrm{btemp} - v(\mathbf{1}) + v(\mathbf{0})}{\mathbf{1}^T \mathrm{Atemp}\inv \mathbf{1}}\Big)$\;
        estimates.append($\beta_m$)\;
        counter = 0\;
        Atemp = 0\;
        btemp = 0\;
        {}\;
        \tcp{Get estimates, uncertainties}
        $\beta_n = \mathrm{A}\inv \Big(\mathrm{b} - \mathbf{1} \frac{\mathbf{1}^T \mathrm{A}\inv \mathrm{b} - v(\mathbf{1}) + v(\mathbf{0})}{\mathbf{1}^T \mathrm{A}\inv \mathbf{1}}\Big)$\;
        $\Sigma_\beta = m \cdot \Cov(\mathrm{estimates})$ {   } \tcp{Empirical covariance}
        $\sigma_n = \sqrt{\mathrm{diag}(\Sigma_\beta) / \mathrm{n}}$ {   } \tcp{Element-wise square root}
        {}\;
        \tcp{Check for convergence}
        converged = $\Big( \frac{\max(\sigma_n)}{\max(\beta_n) - \min(\beta_n)} < t$ \Big)\;
    }
}
\KwRet{$\beta_n$, $\sigma_n$}
\caption{Shapley value estimation with dataset sampling (KernelSHAP)}
\label{alg:kernelshap}
\end{algorithm}


==> Shapley Regression AISTATS 2021 (Camera Ready)/algorithms/kernelshap_stochastic.tex <==
\begin{algorithm}[t]
\SetAlgoLined
\DontPrintSemicolon
\KwIn{Game $V$, convergence threshold $t$, intermediate samples $m$}
\tcp{Initialize}
n = 0\;
A = 0\;
b = 0\;
{}\;
\tcp{For tracking intermediate samples}
counter = 0\;
Atemp = 0\;
btemp = 0\;
estimates = list() \;
{}\;
\tcp{Sampling loop}
converged = False\;
\While{\upshape not converged}{
    \tcp{Draw next sample}
    Sample $z \sim p(Z)$\;
    Sample $u \sim p(U)$\;
    \uIf{\upshape variance reduction}{
        % \textcolor{red}{Need to figure out which version of this estimator works best. Use expectation here?}\;
        bsample = $\frac{1}{2} \big(zV(z, u) + (\mathbf{1} {-} z)V(\mathbf{1} {-} z, u) - \E_U[V(\mathbf{0}, U)]\big)$\;
        Asample = $\frac{1}{2} \big( zz^T + (\mathbf{1} - z)(\mathbf{1} - z)^T \big)$\;
    }
    \uElse{
        bsample = $z \big( V(z, u) - \E_U[V(\mathbf{0}, U)] \big)$\;
        Asample = $zz^T$\;
    }
    {}\;
    \tcp{Welford's algorithm}
    n = n + 1\;
    b += (bsample $-$ b) / n\;
    A += (Asample $-$ A) / n \;
    counter += 1\;
    btemp += (bsample $-$ btemp) / counter\;
    Atemp += (Asample $-$ Atemp) / counter \;
    {}\;
    \uIf{\upshape counter == $m$}{
        \tcp{Get intermediate estimate}
        $\beta_m = \mathrm{Atemp}\inv \Big(\mathrm{btemp} - \mathbf{1} \frac{\mathbf{1}^T \mathrm{Atemp}\inv \mathrm{btemp} - \E_U[V(\mathbf{1}, U)] + \E_U[V(\mathbf{0}, U)]}{\mathbf{1}^T \mathrm{Atemp}\inv \mathbf{1}}\Big)$\;
        estimates.append($\beta_m$)\;
        counter = 0\;
        Atemp = 0\;
        btemp = 0\;
        {}\;
        \tcp{Get estimates, uncertainties}
        $\beta_n = \mathrm{A}\inv \Big(\mathrm{b} - \mathbf{1} \frac{\mathbf{1}^T \mathrm{A}\inv \mathrm{b} - \E_U[V(\mathbf{1}, U)] + \E_U[V(\mathbf{0}, U)]}{\mathbf{1}^T \mathrm{A}\inv \mathbf{1}}\Big)$\;
        $\Sigma_\beta = m \cdot \Cov(\mathrm{estimates})$ {   } \tcp{Empirical covariance}
        $\sigma_n = \sqrt{\mathrm{diag}(\Sigma_\beta) / \mathrm{n}}$ {   } \tcp{Element-wise square root}
        {}\;
        \tcp{Check for convergence}
        converged = $\Big( \frac{\max(\sigma_n)}{\max(\beta_n) - \min(\beta_n)} < t$ \Big)\;
    }
}
\KwRet{$\beta_n$, $\sigma_n$}
\caption{Shapley value estimation with dataset sampling for stochastic cooperative games}
\label{alg:kernelshap_stochastic}
\end{algorithm}


==> Shapley Regression AISTATS 2021 (Camera Ready)/algorithms/unbiased.tex <==
\begin{algorithm}[t]
\SetAlgoLined
\DontPrintSemicolon
\KwIn{Game $v$, convergence threshold $t$}
\tcp{Initialize}
Set $A$ (Section~3.3)\;
Set $C$ (Eq.~13)\;
n = 0\;
b = 0\;
bSSQ = 0\;
{}\;
\tcp{Sampling loop}
converged = False\;
\While{\upshape not converged}{
    \tcp{Draw next sample}
    Sample $z \sim p(Z)$\;
    \uIf{\upshape variance reduction}{
        bsample = $\frac{1}{2} \big(zv(z) + (\mathbf{1} {-} z)v(\mathbf{1} {-} z) - v(\mathbf{0})\big)$\;
    }
    \uElse{
        bsample = $zv(z) - \frac{1}{2}v(\mathbf{0})$\;
    }
    {}\;
    \tcp{Welford's algorithm}
    n = n + 1\;
    diff = (bsample $-$ b) \;
    b += diff / n\;
    diff2 = (bsample $-$ b) \;
    bSSQ += outer(diff, diff2) {   } \tcp{Outer product}\;
    \tcp{Get estimates, uncertainties}
    $\beta_n = A\inv \Big(\mathrm{b} - \mathbf{1} \frac{\mathbf{1}^T A\inv \mathrm{b} - v(\mathbf{1}) + v(\mathbf{0})}{\mathbf{1}^T A\inv \mathbf{1}}\Big)$\;
    $\Sigma_{b} = $ bSSQ / n\;
    $\Sigma_{\beta} = C \Sigma_{b} C^T$\;
    $\sigma_n = \sqrt{\mathrm{diag}(\Sigma_{\beta}) / \mathrm{n}}$ {   } \tcp{Element-wise square root} \;
    \tcp{Check for convergence}
    converged = $\Big( \frac{\max(\sigma_n)}{\max(\beta_n) - \min(\beta_n)} < t$ \Big)\;
}
\KwRet{$\beta_n$, $\sigma_n$}
\caption{Unbiased Shapley value estimation}
\label{alg:unbiased}
\end{algorithm}


==> Shapley Regression AISTATS 2021 (Camera Ready)/algorithms/unbiased_stochastic.tex <==
\begin{algorithm}[t]
\SetAlgoLined
\DontPrintSemicolon
\KwIn{Game $V$, convergence threshold $t$}
\tcp{Initialize}
Set $A$ (Section~3.3)\;
Set $C$ (Eq.~13)\;
n = 0\;
b = 0\;
bSSQ = 0\;
{}\;
\tcp{Sampling loop}
converged = False\;
\While{\upshape not converged}{
    \tcp{Draw next sample}
    Sample $z \sim p(Z)$\;
    Sample $u \sim p(U)$\;
    \uIf{\upshape variance reduction}{
        bsample = $\frac{1}{2} \Big(zV(z, u) + (\mathbf{1} {-} z)V(\mathbf{1} {-} z, u) - \E_U\big[ V(\mathbf{0}), U \big] \Big)$\;
    }
    \uElse{
        bsample = $zV(z, u) - \frac{1}{2} \E_U[V(\mathbf{0}, U)]$\;
    }
    {}\;
    \tcp{Welford's algorithm}
    n = n + 1\;
    diff = (bsample $-$ b) \;
    b += diff / n\;
    diff2 = (bsample $-$ b) \;
    bSSQ += outer(diff, diff2) {   } \tcp{Outer product}\;
    \tcp{Get estimates, uncertainties}
    $\beta_n = A\inv \Big(\mathrm{b} - \mathbf{1} \frac{\mathbf{1}^T A\inv \mathrm{b} - \E_U[V(\mathbf{1}, U)] + \E_U[V(\mathbf{0}, U)]}{\mathbf{1}^T A\inv \mathbf{1}}\Big)$\;
    $\Sigma_{b} = $ bSSQ / n\;
    $\Sigma_{\beta} = C \Sigma_{b} C^T$\;
    $\sigma_n = \sqrt{\mathrm{diag}(\Sigma_{\beta}) / \mathrm{n}}$ {   } \tcp{Element-wise square root} \;
    \tcp{Check for convergence}
    converged = $\Big( \frac{\max(\sigma_n)}{\max(\beta_n) - \min(\beta_n)} < t$ \Big)\;
}
\KwRet{$\beta_n$, $\sigma_n$}
\caption{Unbiased Shapley value estimation for stochastic cooperative games}
\label{alg:unbiased_stochastic}
\end{algorithm}


==> Shapley Regression AISTATS 2021 (Camera Ready)/inserts/acceleration.tex <==
\begin{figure} % [ht]
% \vskip 0.2in
\begin{center}
\includegraphics[trim=0.8cm 0cm 0.4cm 0.2cm, clip=true, width=\columnwidth]{images/acceleration_joint.pdf}
\vskip -0.2in
\caption{Convergence acceleration for SAGE and Shapley Effects. The ratio of the maximum standard deviation to the gap between the largest and smallest Shapley values is compared across six estimators.}
\label{fig:acceleration}
\end{center}
\vskip -0.2in
\end{figure}

==> Shapley Regression AISTATS 2021 (Camera Ready)/inserts/bank_mse.tex <==
\begin{figure} % [ht]
\begin{center}
\includegraphics[width=\columnwidth]{images/bank_error_grid.pdf}
% \vskip -0.2in
\caption{Bank marketing SHAP value estimation error on four predictions.}
\label{fig:bank_mse}
\vskip 0.5in
\includegraphics[width=\columnwidth]{images/bank_variance_rate.pdf}
\caption{Bank marketing SHAP value variance estimation on four predictions.}
\label{fig:bank_variance}
\end{center}
\end{figure}

==> Shapley Regression AISTATS 2021 (Camera Ready)/inserts/bias-variance.tex <==
% \begin{table*}
% \caption{Global measures of bias and variance for each SHAP value estimator. Each entry is the mean bias and mean variance calculated empirically across 100 examples (\textit{bias}/\textit{variance}, lower is better).}
% \label{tab:bias_variance}
% \vskip 0.1in
% \begin{center}
% \begin{small}
% \begin{tabular}{lccc}
% \toprule
%  & \textsc{Census Income} & \textsc{Bank Marketing} & \textsc{German Credit} \\
% \midrule
% Unbiased & 0.0000/0.0026 & 0.0000/0.0016 & 0.0001/0.0322 \\
% Unbiased + Paired Sampling & 0.0000/0.0008 & 0.0000/0.0008 & 0.0001/0.0008 \\
% Original (KernelSHAP) & 0.0000/0.0001 & 0.0000/0.0001 & 0.0001/0.0000 \\
% Original + Paired Sampling & 0.0000/0.0000 & 0.0000/0.0000 & 0.0001/0.0000 \\
% \bottomrule
% \end{tabular}
% \end{small}
% \end{center}
% \end{table*}


\begin{table*}
\caption{Global measures of bias and variance for each SHAP value estimator. Each entry is the mean bias and mean variance calculated empirically across 100 examples (bias/variance, lower is better).}
\label{tab:bias_variance}
\vskip 0.1in
\begin{center}
\begin{small}
\begin{tabular}{lccc}
\toprule
 & \textsc{Census Income} & \textsc{Bank Marketing} & \textsc{German Credit} \\
\midrule
Unbiased & 0.0002/0.0208 & 0.0001/0.0125 & 0.0026/0.2561 \\
Unbiased + Paired Sampling & 0.0000/0.0068 & 0.0000/0.0066 & 0.0000/0.0062 \\
Original (KernelSHAP) & 0.0000/0.0007 & 0.0000/0.0006 & 0.0000/0.0002 \\
Original + Paired Sampling & 0.0000/0.0001 & 0.0000/0.0001 & 0.0000/0.0000 \\
\bottomrule
\end{tabular}
\end{small}
\end{center}
\end{table*}


==> Shapley Regression AISTATS 2021 (Camera Ready)/inserts/census_mse.tex <==
\begin{figure} % [ht]
\begin{center}
\includegraphics[width=\columnwidth]{images/census_error_grid.pdf}
% \vskip -0.2in
\caption{Census income SHAP value estimation error on four predictions.}
\label{fig:census_mse}
\vskip 0.5in
\includegraphics[width=\columnwidth]{images/census_variance_rate.pdf}
\caption{Census income SHAP value variance estimation on four predictions.}
\label{fig:census_variance}
\end{center}
\end{figure}

==> Shapley Regression AISTATS 2021 (Camera Ready)/inserts/confidence.tex <==
\begin{figure} % [ht]
% \vskip 0.2in
\begin{center}
\includegraphics[width=\columnwidth]{images/confidence_ellipsoid.pdf}
\vskip -0.2in
\caption{Gaussian 95\% confidence ellipsoids for two SHAP values in a census income prediction (from 250 runs).
The estimators use
% Each estimator uses
an equal
% a fixed
number of samples.}
\label{fig:confidence}
\end{center}
\vskip -0.2in
\end{figure}

==> Shapley Regression AISTATS 2021 (Camera Ready)/inserts/credit_mse.tex <==
\begin{figure} % [ht]
\begin{center}
\includegraphics[width=\columnwidth]{images/credit_error_grid.pdf}
% \vskip -0.2in
\caption{German credit SHAP value estimation error on four predictions.}
\label{fig:credit_mse}
\vskip 0.5in
\includegraphics[width=\columnwidth]{images/credit_variance_rate.pdf}
\caption{German credit SHAP value variance estimation on four predictions.}
\label{fig:credit_variance}
\end{center}
\end{figure}

==> Shapley Regression AISTATS 2021 (Camera Ready)/inserts/error.tex <==
\begin{figure} % [ht]
% \vskip 0.2in
\begin{center}
\includegraphics[width=\columnwidth]{images/error_decomposition.pdf}
\vskip -0.2in
\caption{SHAP error decomposition for the original and unbiased KernelSHAP estimators. The bias and variance are calculated empirically across 250 runs.}
\label{fig:error}
\end{center}
\vskip -0.1in
\end{figure}

==> Shapley Regression AISTATS 2021 (Camera Ready)/inserts/forecasting.tex <==
\begin{figure} % [ht]
% \vskip 0.2in
\begin{center}
\includegraphics[trim=1.4cm 1.1cm 0.5cm 0.5cm, clip=true, width=\columnwidth]{images/forecasting.pdf}
% \vskip -0.25in
\caption{Convergence forecasting for SHAP, Shapley Effects and SAGE. The required number of samples is compared with the predicted number across 100 runs (with 90\% confidence intervals displayed).}
\label{fig:forecasting}
\end{center}
\vskip -0.2in
\end{figure}

==> Shapley Regression AISTATS 2021 (Camera Ready)/inserts/shap_comparison.tex <==
\begin{table*}
\caption{SHAP estimator run-time comparison. Each value represents the ratio of the average number of samples required relative to the fastest estimator for that dataset (lower is better).}
\label{tab:shap_comparison}
\vskip 0.1in
\begin{center}
\begin{small}
\begin{tabular}{lcccc}
\toprule
 & \textsc{Census Income} & \textsc{Bank Marketing} & \textsc{German Credit} & \textsc{BRCA Subtypes} \\
\midrule
Unbiased & 380.63 & 176.45 & 17437.44 & 90.40 \\
Unbiased + Paired Sampling & 128.60 & 90.61 & 422.17 & 40.44 \\
Original (KernelSHAP) & 12.74 & 7.41 & 13.74 & 2.49 \\
Original + Paired Sampling & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} & \textbf{1.00} \\
\bottomrule
\end{tabular}
\end{small}
\end{center}
\end{table*}


==> Shapley Regression AISTATS 2021 (Camera Ready)/math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> Shapley Regression AISTATS 2021 (Camera Ready)/old/body.tex <==
\section{Introduction}

KernelSHAP is one of the most popular methods for estimating SHAP values, which are the Shapley values of a cooperative game representing an individual prediction. The method is based on Scott's observation that Shapley values are the solution to a weighted constrained linear regression problem.

Despite KernelSHAP's popularity, I expect that many people don't understand how it works. I'm one of those people. But I need to understand it to implement it for my Shapley value estimation implementations (particularly SAGE). In these notes, I'll derive how to estimate a cooperative game's Shapley values by solving a constrained least squares problem.

\section{Linear Regression}

A linear regression model with data points $(x_i, y_i)$ for $i = 1, 2, \ldots, n$ is fit by solving the following least squares problem:

\begin{align*}
    \sum_{i=1}^n (x-i^T \beta + \beta_0 - y_i)
    &= ||X\beta + \mathbf{1}\beta_0 - Y||^2 \\
    &= ||\begin{pmatrix}\mathbf{1} & X \end{pmatrix} \begin{pmatrix} \beta_0 \\ \beta \end{pmatrix} - Y||^2
\end{align*}

A weighted least squares problem is given by the following:

\begin{align*}
    \Big(\begin{pmatrix}\mathbf{1} & X \end{pmatrix} \begin{pmatrix} \beta_0 \\ \beta \end{pmatrix} - Y\Big)^T W \Big(\begin{pmatrix}\mathbf{1} & X \end{pmatrix} \begin{pmatrix} \beta_0 \\ \beta \end{pmatrix} - Y\Big)
\end{align*}

where $W$ is a diagonal matrix with entries specifying the weights for each data point.

Shapley values are based on solving a weighted least squares problem, with weights given by the ``Shapley kernel,'' as it is informally known. However, we won't be able to solve it as a weighted least squares problem because we can't obtain all the necessary data points. Instead, we'll re-express the objective as an expectation over a distribution.

\begin{align*}
    \sum_{i = 1}^n w_i (x_i^T \beta + \beta_0 - y_i)^2
    &= \E[(X^T \beta + \beta_0 - Y)]
\end{align*}

In the above, capital letters refer to random variables rather than matrices (as in the linear algebra equations further above). Now, we can estimate this objective by sampling $x$ according to the distribution induces by the weights $w_i$.

\begin{align*}
    \E[(X^T \beta + \beta_0 - Y)]
    &\approx \frac{1}{n} \sum_{i = 1}^n (x_i^T \beta + \beta_0 - y_i)^2 \\
    &= \frac{1}{n} ||\begin{pmatrix}\mathbf{1} & X \end{pmatrix} \begin{pmatrix} \beta_0 \\ \beta \end{pmatrix} - Y||^2
\end{align*}

where $X, Y$ are now matrices containing the samples $x_i, y_i$. This can be understood as a stochastic estimator of the true objective. If we expand it we can see that it's consistent:

\begin{align*}
    \frac{1}{n} \Big(\begin{pmatrix} \beta_0 \\ \beta \end{pmatrix}^T \begin{pmatrix}\mathbf{1} & X \end{pmatrix}^T \begin{pmatrix}\mathbf{1} & X \end{pmatrix} \begin{pmatrix} \beta_0 \\ \beta \end{pmatrix}
    - 2 Y^T \begin{pmatrix}\mathbf{1} & X \end{pmatrix} \begin{pmatrix} \beta_0 \\ \beta \end{pmatrix}
    + Y^TY \Big)
\end{align*}

It's consistent because the two variance and the one covariance term are consistent estimators. It's not quite unbiased, but I think it could be made unbiased with a simple modification of $\frac{1}{n}$ to $\frac{1}{n - 1}$. This isn't important, we're not as focused on our estimator of the objective as we are on the problem's solution.

Solving this problem is pretty easy when we use matrix derivatives. But unfortunately, the Shapley problem is even more complicated than this because it incorporates constraints.

When Shapley values are expressed as the solution to a weighted least squares problem, it has two constraints:

\begin{align*}
    \beta_0 &= v(\varnothing) \\
    \sum_{i = 1}^d \beta_i &= v(D) - v(\varnothing)
\end{align*}

In our case, if we sample data points according to some distribution that matches the Shapley kernel conditioned on points being included, then we can simply partition our samples into three sets: 1) those where all features are included, 2) those where no features are included, 3) those where some features are included. Then we can use this to estimate constants corresponding to the constraints. TODO come back to this

The Shapley kernel is the following:

\begin{align*}
    \pi(S) = \frac{d - 1}{\binom{d}{|S|}|S|(d - |S|)}
\end{align*}

Now, for $S$ such that $0 < |S| < d$ (the prediction is not fixed by constraints), we have:

\begin{align*}
    \pi(S) &= \frac{(|S| - 1)!(d - |S| - 1)!}{(d - 1)!} \\
    &= \frac{1}{d - 1} \binom{d - 2}{|S| - 1}\inv
\end{align*}

This is consistent with the kernel described by Charnes at al., at least according to Hammer and Holtzman (since I can't access the Charnes paper). Now, I must figure out how to sample from a distribution that's close to this.

\clearpage

\section{Regression-Based Estimates for Shapley Values}

Here's an easier way to think about this. We have a cooperative game $v: \mathcal{P}(D) \mapsto \R$, and with abuse of notation we can think of this as a function $v: \{0, 1\}^d \mapsto \R$. The input coalitions $S \subseteq D$ can be represented as binary vectors $x \in \{0, 1\}^d$, and we can imagine fitting a weighted linear model as follows:

\begin{align*}
    \sum_{x} w(x) \big(\beta_0 + \sum_{i = 1}^d x_i \beta_i - v(x)\big)^2
\end{align*}

The Shapley value can be expressed as a solution to one of these problems, but with a kernel that effectively puts constraints on $\beta_0, \ldots, \beta_d$. The problem looks like the following:

\begin{align*}
    &\sum_{x} \pi(x) \big(\beta_0 + \sum_{i=1}^d x_i \beta_i - v(c) \big) \\
    &\mathrm{s.t.} \quad \beta_0 = v(\{\}), \quad \sum_{i = 1}^d \beta_i = v(D) - v(\{\})
\end{align*}

where the weighting kernel is given by

\begin{align*}
    \pi(x) = \begin{cases}
        \binom{d-2}{|S| - 1}\inv \quad\quad 0 < \mathbf{1}^Tx < d \\
        0 \quad\quad \mathrm{else}
    \end{cases}
\end{align*}

For large values of $d$, we won't be able to calculate this full objective or obtain the closed-form solution. Instead, we find the exact solution to an approximate version of the objective, and sample $x$'s according to the distribution induced by $\pi$. Our approximate objective is:

\begin{align*}
    &\frac{1}{n} \sum_{i = 1}^n \big(\beta_0 + \sum_{j = 1}^d x_{ij} \beta_j - v(x_i) \big)^2 \\
    &\mathrm{s.t.} \quad \beta_0 = v(\{\}), \quad \sum_{i = 1}^d \beta_i = v(D) - v(\{\})
\end{align*}

Solving this problem is much more manageable. We rewrite it by denoting $\beta = (\beta_1, \ldots, \beta_d)$ and using matrix notation:

\begin{align*}
    &\frac{1}{n} ||X \beta - (Y - \mathbf{1} \beta_0)||^2 \\
    &\mathrm{s.t.} \quad \beta_0 = v(\{\}), \quad \sum_{i = 1}^d \beta_i = v(D) - v(\{\})
\end{align*}

where $Y_i = v(x_i)$. We can find a closed form solution to this problem by solving the Lagrangian:

\begin{align*}
    \mathcal{L}(\beta, \lambda) &= \frac{1}{n}||X \beta - (Y - \mathbf{1} \beta_0)||^2 + 2 \lambda (\mathbf{1}^T \beta - v(D) + v(\{\}))
\end{align*}

If we take the derivative with respect to $\beta$ we get:

\begin{align*}
    \frac{\partial \mathcal{L}}{\partial \beta}(\beta, \lambda) = 2 \big(\frac{1}{n} X^TX\big) \beta - 2 \Big(\frac{1}{n}X^T \big(Y - \mathbf{1}v(\{\})\big) \Big) + 2 \mathbf{1}\lambda
\end{align*}

This yields the closed-form solution:

\begin{align*}
    \beta^* = \big(\frac{1}{n} X^TX\big)\inv \Big(\frac{1}{n} X^T \big(Y - \mathbf{1}v(\{\})\big) - \mathbf{1}\lambda \Big)
\end{align*}

The only remaining question is, what value does the dual variable $\lambda$ take for the optimal solution? We can find this by using the fact that the constraint must hold:

\begin{align*}
    \mathbf{1}^T \beta^* = v(D) - v(\{\})
\end{align*}

This gives us the following equation for $\lambda$:

\begin{align*}
    \lambda = \Big[\mathbf{1}^T \big(\frac{1}{n} X^TX\big)\inv (\frac{1}{n} X^T \big(Y - \mathbf{1}v(\{\})\big) - \big(v(D) - v(\{\})\big) \Big] / \Big(\mathbf{1}^T \big(\frac{1}{n} X^TX\big)\inv \mathbf{1}\Big)
\end{align*}

And finally, this gives us the following solution for $\beta^*$:

\begin{align*}
    \beta^* = \; &\big(\frac{1}{n} X^TX\big)\inv \frac{1}{n} X^T \big(Y - \mathbf{1}v(\{\})\big) \\
    &- \Big(\mathbf{1}^T \big(\frac{1}{n} X^TX\big)\inv \mathbf{1}\Big)\inv \big(\frac{1}{n} X^TX\big)\inv \mathbf{1}\Big(\mathbf{1}^T \big(\frac{1}{n} X^TX\big)\inv (\frac{1}{n} X^T \big(Y - \mathbf{1}v(\{\})\big) - \big(v(D) - v(\{\})\big) \Big)
\end{align*}

We can simplify this by denoting the following quantities:

\begin{align*}
    A &= \frac{1}{n}X^TX \\
    b &= \frac{1}{n} X^TY \\
    c &= \frac{1}{n} X^T \mathbf{1} \\
    a_0 &= v(\{\}) \\
    a_1 &= v(D) - v(\{\})
\end{align*}

This allows us to rewrite the solution as:

\begin{align*}
    \beta^* = A\inv (b - ca_0) - (\mathbf{1}^T A\inv \mathbf{1})\inv A\inv \mathbf{1} \Big(\mathbf{1}^T A\inv (b - ca_0) - a_1\Big)
\end{align*}

We can remove certain sources of stochasticity from this estimator by using the exact form for a couple of these terms. In particular, the following quantities can be calculated exactly using the distribution induced by $\pi$:

\begin{align*}
    \E[A_{ij}] &= p(i, j \in S) \\
    \E[c_i] &= p(i \in S)
\end{align*}

These can be calculated exactly, but they require us to consider the distribution over subsets more carefully. The distribution induced by $\pi$ for $S$ such that $0 < |S| < d$ is

\begin{align*}
    p(S) = \alpha \binom{d - 2}{|S| - 1}\inv
\end{align*}

which means that $\alpha$ is given by

\begin{align*}
    \alpha\inv &= \sum_{0 < |S| < d} \binom{d - 2}{|S| - 1}\inv \\
    &= \sum_{k = 1}^{d - 1} \binom{d}{k} \binom{d - 2}{k - 1}\inv \\
    &= \sum_{k = 1}^{d - 1} \frac{d!}{k!(d-k)!} \frac{(k-1)!(d-k-1)!}{(d-2)!} \\
    &= \sum_{k=1}^{d-1} \frac{d(d-1)}{k(d-k)}
\end{align*}

Now, we can see that the exact values for $\E[c]$ is given by:

\begin{align*}
    \E[c_i] &= p(i \in S) \\
    &= \sum_{k = 1}^{d-1} p(i \in S \; | \; |S| = k) p(|S| = k) \\
    &= \alpha \sum_{k = 1}^{d-1} \binom{d - 1}{k - 1}\binom{d}{k}\inv \cdot \binom{d}{k} \binom{d - 2}{k - 1}\inv \\
    &= \alpha \sum_{k = 1}^{d - 1} \frac{d - 1}{d - k} \\
    &= \frac{\sum_{k = 1}^{d - 1} \frac{d - 1}{d - k}}{\sum_{k=1}^{d-1} \frac{d(d-1)}{k(d-k)}}
\end{align*}

We can prove that this is equal to $\frac{1}{2}$ as follows:

\begin{align*}
    1 - \E[c_i] &= 1 - \frac{\sum_{k = 1}^{d - 1} \frac{d - 1}{d - k}}{\sum_{k=1}^{d-1} \frac{d(d-1)}{k(d-k)}} \\
    &= \Big( \sum_{k=1}^{d-1} \frac{d(d-1)}{k(d-k)} \Big)\inv \Big(\sum_{k=1}^{d-1} \frac{d(d-1)}{k(d-k)} - \sum_{k = 1}^{d - 1} \frac{d - 1}{d - k} \Big) \\
    &= \Big( \sum_{k=1}^{d-1} \frac{d(d-1)}{k(d-k)} \Big)\inv \Big(\sum_{k=1}^{d-1} \frac{d(d-1)}{k(d-k)} - \frac{k(d - 1)}{k(d - k)} \Big) \\
    &= \frac{\sum_{k = 1}^{d - 1} \frac{d - 1}{d - k}}{\sum_{k=1}^{d-1} \frac{d(d-1)}{k(d-k)}} \\
    &= \E[c_i] \\
    &\Rightarrow \E[c_i] = \frac{1}{2}
\end{align*}

Now, we can do a similar analysis for $\E[A_{ij}]$. First, we can see that diagonal entries have the following expectation:

\begin{align*}
    \E[A_{ii}] &= p(i \in S) \\
    &= \E[c_i] \\
    &= \frac{1}{2}
\end{align*}

Off-diagonal entries have the following expectation:

\begin{align*}
    \E[A_{ij}] &= p(i, j \in S) \\
    &= \sum_{k = 2}^{d - 1} p(i, j \in S \; | \; |S| = k) p(|S| = k) \\
    &= \alpha \sum_{k = 2}^{d - 1} \binom{d - 2}{k - 2} \binom{d}{k}\inv \cdot \binom{d}{k} \binom{d - 2}{k - 1}\inv \\
    &= \alpha \sum_{k = 2}^{d - 1} \frac{k - 1}{d - k} \\
    &= \frac{\sum_{k = 2}^{d - 1} \frac{k - 1}{d - k}}{\sum_{k=1}^{d-1} \frac{d(d-1)}{k(d-k)}}
\end{align*}

It doesn't seem like there's a convenient way to simplify this, but we can calculate it numerically for a given value of $d$.

Anyway, this approach shows how to estimate Shapley values by calculating the exact solution to an approximate problem.

\section{An Approximate Solution to the Exact Problem}

Rather than stochastically estimating the objective and then optimizing the approximate objective, let's revisit the true objective:

\begin{align*}
    &\E_{p(S)}\Big[\big(\beta_0 + \sum_{i = 1}^d x_i(S) \beta_i - v(x(S))\big)\Big] \\
    &\mathrm{s.t.} \quad \beta_0 = v(\{\}), \quad \sum_{i = 1}^d \beta_i = v(D) - v(\{\})
\end{align*}

Now, write this using matrix algebra:

\begin{align*}
    % \mathcal{L}(\beta_0, \ldots, \beta_d) &=
    &\; \E_{p(S)}\Big[\big(\beta_0 + \sum_{i = 1}^d x_i(S) \beta_i - v(x(S))\big)\Big] \\
    % &= \E_{p(S)} \Big[ \big(\begin{pmatrix}1 & x \end{pmatrix} \begin{pmatrix} \beta_0 \\ \beta \end{pmatrix} - v(x(S))\big)^2 \Big] \\
    &= \E_{p(S)} \Big[ \big(x^T \beta  - (v(x(S)) - \beta_0)\big)^2 \Big] \\
    &= \E_{p(S)} \Big[ \big(x^T \beta  - (y(x) - \beta_0)\big)^2 \Big] \\
    &= \E_{p(S)} \Big[ \beta^T x x^T \beta - 2 \beta^T x (y(x) - \beta_0) + (y(x) - \beta_0)^2 \Big] \\
    &= \beta^T \E[xx^T] \beta - 2 \beta^T \E[xy(x)] + \E[(y(x) - \beta_0)^2]
\end{align*}

If we use this version of the objective function and write the problem's Lagrangian, we get the following:

\begin{align*}
    \mathcal{L}(\beta, \lambda) = \beta^T \E[xx^T] \beta - 2 \beta^T \E[xy(x)] + \E[(y(x) - \beta_0)^2] + 2\lambda (\mathbf{1}^T \beta - (v(D) - v(\{\})))
\end{align*}

If we solve this, we get the same solution as above, but with $A, b, c$ substituted with their expectations. If we use the exact forms for $\E[A], \E[c]$ and just estimate $b$, then we see how this is an estimator for the solution $\beta^*$ to the true objective.

We can even make a couple remarks about the estimator. The first is that it's consistent, because obviously. The second is that it's unbiased, because the mean is clearly the true value (linear dependence on the only thing being estimated). The third is that the multivariate central limit theorem (MCLT) says that our $b$ estimator asymptotically has a multivariate Gaussian distribution; the estimator therefore asympototically has a multivariate Gaussian distribution. If we estimate $b$'s covariance, then we estimate the estimator's covariance. We use this for providing uncertainty estimates (the diagonal entries) and detecting convergence automatically.

\section{What's Next}

I've found that for SAGE and Shapley Effects, which are for our purposes two stochastic cooperative games, the regression approach has significantly higher variance than the permutation sampling approach. I'm confident in my derivation, and I have empirical evidence that my implementation is correct, so the logical conclusion is that this algorithm simply suffers from higher variance than the permutation sampling algorithm. This was unexpected, because Figure 3 of Scott's NeurIPS paper made it seem like KernelSHAP has way lower variance than IME. 

If Scott was right about KernelSHAP being faster than IME, than maybe I can implement my uncertainty estimates in the removal-based explanations package and see that it 1) gives previously non-existent uncertainty estimates, 2) that it runs faster than the sampling algorithm.

Unfortunately, I haven't really implemented KernelSHAP. I implemented an unregularized constrained least squares problem, but KernelSHAP allows for regularizers. I can get a closed form solution for the ridge version, but not for the Lasso version. What do I do now? I think I need to find an analysis of the variance of a Lasso estimator. These slides are my best hope, they have a shitty variance estimator: \url{http://www.few.vu.nl/~wvanwie/Courses/HighdimensionalDataAnalysis/WNvanWieringen_HDDA_Lecture56_LassoRegression_20182019.pdf}. For $\lambda > 0$ this better yield lower variance than we would get with $\lambda = 0$.

Even if I can figure out how to quantify variance for both types of regularization, I'll have to think about incorporating different weighting kernels (e.g., cosine, uniform). I think that's easy enough: just calculate the weights vector numerically, and then calculate $\E[A]$ and $\E[c]$ numerically.

Then, the last thing to figure out will be how to choose the regularization parameter. For Lasso, people might want to specify the number of non-zero regression coefficients; but what about for Ridge? (That one is interesting to me because it will be easier for me to implement, since closed form solution is almost the same). The usual answer (use cross validation) doesn't work here, because we don't have a validation dataset. In fact, we don't have a dataset at all because I'm only keeping track of sufficient statistics.

I implemented the Ridge penalty and it still didn't fix my problem. It's one thing for the confidence intervals to scale uniformly across the different features, regardless of the SAGE value. But it's another for the largest confidence interval to shrink more slowly than it does with permutation sampling. I'm abandoning this now for SAGE, it does not appear to work.

I thought the derivations were cool, but it's all for nothing if this method is pointless. The only case I can come up with where it's not pointless is for SHAP, where the NeurIPS paper claims it's better than sampling. But that experiment is lacking a lot of details so it's hard to say for sure.

==> Shapley Regression AISTATS 2021 (Camera Ready)/supp_content.tex <==
% \onecolumn

\section[alternative title]{CALCULATING $A$ EXACTLY} \label{app:exact}

Recall the definition of $A$, which is a term in the solution to the Shapley value linear regression problem:

\begin{equation*}
    A = \E[ZZ^T].
\end{equation*}

The entries of $A$ are straightforward to calculate because $Z$ is a random binary vector with a known distribution. Recall that $Z$ is distributed according to $p(Z)$, which is defined as:

\begin{align*}
    p(z) = \begin{cases}
        Q\inv \mu_{\mathrm{Sh}}(Z) \quad 0 < \mathbf{1}^Tz < d \\
        0 \quad\quad\quad\quad\quad\; \mathrm{otherwise},
    \end{cases}
\end{align*}

where the normalizing constant $Q$ is given by:

\begin{align*}
    Q &= \sum_{0 < \mathbf{1}^Tz < d} \mu_{\mathrm{Sh}}(z) \\
    % &= \sum_{0 < \mathbf{1}^Tz < d} \frac{d - 1}{\binom{d}{\mathbf{1}^Tz}(\mathbf{1}^Tz)(d - \mathbf{1}^Tz)} \\
    % &= \sum_{0 < \mathbf{1}^Tz < d} \frac{d - 1}{\binom{d}{\mathbf{1}^Tz}d(d - \mathbf{1}^Tz)} \\
    &= \sum_{k = 1}^{d - 1} \binom{d}{k} \frac{d - 1}{\binom{d}{k}k(d - k)} \\
    &= (d - 1) \sum_{k = 1}^{d - 1} \frac{1}{k(d - k)}.
\end{align*}

Although $Q$ does not have a simple closed-form solution, the expression above can be calculated numerically. The diagonal entries $A_{ii}$ are then given by:

\begin{align*}
    A_{ii} &= \E[Z_iZ_i]
    = p(Z_i = 1) \\
    &= \sum_{k = 1}^{d - 1} p(Z_i = 1 | \mathbf{1}^TZ = k) p(\mathbf{1}^TZ = k) \\
    &= \sum_{k = 1}^{d - 1} \frac{\binom{d - 1}{k - 1}}{\binom{d}{k}} \cdot Q\inv \binom{d}{k} \frac{d - 1}{\binom{d}{k}k(d - k)} \\
    % &= \frac{1}{(d - 1) \sum_{k = 1}^{d - 1} \frac{1}{k(d - k)}} \sum_{k = 1}^{d - 1} \frac{d - 1}{d(d - k)} \\
    &= \frac{\sum_{k = 1}^{d - 1} \frac{1}{d(d - k)}}{\sum_{k = 1}^{d - 1} \frac{1}{k(d - k)}}.
\end{align*}

This is equal to $\frac{1}{2}$ regardless of the value of $d$. To see this, consider the probability $p(Z_i = 0)$:

\begin{align*}
    p(Z_i = 0) &= 1 - p(Z_i = 1) \\
    &= 1 - \frac{\sum_{k = 1}^{d - 1} \frac{1}{d(d - k)}}{\sum_{k = 1}^{d - 1} \frac{1}{k(d - k)}} \\
    % &= \frac{\sum_{k = 1}^{d - 1} \frac{1}{k(d - k)} - \sum_{k = 1}^{d - 1} \frac{1}{d(d - k)}}{\sum_{k = 1}^{d - 1} \frac{1}{k(d - k)}} \\
    % &= \frac{\sum_{k = 1}^{d - 1} \frac{d}{dk(d - k)} - \sum_{k = 1}^{d - 1} \frac{k}{dk(d - k)}}{\sum_{k = 1}^{d - 1} \frac{1}{k(d - k)}} \\
    &= \frac{\sum_{k = 1}^{d - 1} \frac{1}{d(d - k)}}{\sum_{k = 1}^{d - 1} \frac{1}{k(d - k)}} \\
    &= p(Z_i = 1) \\
    % \Rightarrow p(Z_i = 1) + p(Z_i = 0) &= 2p(Z_i = 1) \\
    % &= 1 \\
    \Rightarrow A_{ii} &= \frac{1}{2}.
\end{align*}

Next, consider the off-diagonal entries $A_{ij}$ for $i \neq j$:

\begin{align*}
    A_{ij} &= \E[Z_iZ_j]
    = p(Z_i = Z_j = 1) \\
    &= \sum_{k = 2}^{d - 1} p(Z_i = Z_j = 1 | \mathbf{1}^TZ = k) p(\mathbf{1}^TZ = k) \\
    &= \sum_{k = 2}^{d - 1} \frac{\binom{d - 2}{k - 2}}{\binom{d}{k}} \cdot Q\inv \binom{d}{k} \frac{d - 1}{\binom{d}{k}k(d - k)} \\
    % &= \frac{1}{(d - 1) \sum_{k = 1}^{d - 1} \frac{1}{k(d - k)}} \sum_{k = 2}^{d - 1} \frac{k - 1}{d(d - k)} \\
    &= \frac{1}{d(d - 1)}\frac{\sum_{k = 2}^{d - 1} \frac{k - 1}{d - k}}{\sum_{k = 1}^{d - 1} \frac{1}{k(d - k)}}.
\end{align*}

The value for off-diagonal entries $A_{ij}$ depends on $d$, unlike the diagonal entries $A_{ii}$. Although it does not have a simple closed-form expression, this value can be calculated numerically in $\mathcal{O}(d)$ time.

\section{VARIANCE REDUCTION PROOF} \label{app:variance_reduction}

We present a proof for Theorem~\ref{thm:confidence}, and we prove that a weaker condition than $G_v \succeq 0$ holds for all cooperative games (the diagonal elements satisfy $(G_v)_{ii} \geq 0$ for all games $v$).

\subsection{Theorem~\ref{thm:confidence} Proof}

% We propose
In Section~\ref{sec:var_reduction}, we proposed a variance reduction technique that pairs each sample $z_i \sim p(Z)$ with its complement $\mathbf{1} - z_i$ when estimating $b$. We now provide a proof for the condition that must be satisfied for the estimator $\check \beta_n$ to have lower variance than $\bar \beta_n$. As mentioned in the main text, the multivariate CLT asserts that

\begin{align*}
    \bar b_n \sqrt{n} &\xrightarrow{D} \mathcal{N}(b, \Sigma_{\bar b}) \\
    \check b_n \sqrt{n} & \xrightarrow{D} \mathcal{N}(b, \Sigma_{\check b}),
\end{align*}

where

\begin{align*}
    % \Sigma_{\bar b} &= \Cov\Big(Z \big(v(Z) - v(\mathbf{0})\big)\Big) \\
    % \Sigma_{\check b} &= \Cov\Big(\frac{1}{2} \big(Zv(Z) + (\mathbf{1} - Z)v(\mathbf{1} - Z) - v(\mathbf{0}) \big)\Big).
    \Sigma_{\bar b} &= \Cov\big(Z v(Z)\big), \\
    \Sigma_{\check b} &= \Cov\Big(\frac{1}{2} \big(Zv(Z) + (\mathbf{1} - Z)v(\mathbf{1} - Z) \big)\Big).
\end{align*}

We can also apply the multivariate CLT to the Shapley value estimators $\bar \beta_n$ and $\check \beta_n$. We can see that

\begin{align*}
    \bar \beta_n \sqrt{n} &\xrightarrow{D} \mathcal{N}(\beta^*, \Sigma_{\bar \beta}) \\
    \check \beta_n \sqrt{n} &\xrightarrow{D} \mathcal{N}(\beta^*, \Sigma_{\check \beta}),
\end{align*}

% where we have
where, due to their multiplicative dependence on $b$ estimators, the covariance matrices are defined as

\begin{align*}
    \Sigma_{\bar \beta} &= C \Sigma_{\bar b} C^T \\
    \Sigma_{\check \beta} &= C \Sigma_{\check b} C^T.
\end{align*}

Next, we examine the relationship between $\Sigma_{\bar b}$ and $\Sigma_{\check b}$ because they dictate the relationship between $\Sigma_{\bar \beta}$ and $\Sigma_{\check \beta}$. To simplify our notation, we introduce three jointly distributed random variables, $M^0$, $M^1$ and $\bar M$, which are all functions of the random variable $Z$:

\begin{align*}
    M^0 &= Z v(Z) - \E[Z] v(\mathbf{0}) \\
    M^1 &= (\mathbf{1} - Z) v(\mathbf{1} - Z) - \E[\mathbf{1} - Z] v(\mathbf{0}) \\
    \bar M &= \frac{1}{2} \big( M^0 + M^1 \big).
\end{align*}

To understand $\bar M$'s covariance structure, we can decompose it using standard covariance properties and the fact that $p(z) = p(\mathbf{1} - z)$ for all $z$:

\begin{align*}
    \Cov(\bar M, \bar M)_{ij} &= \frac{1}{4} \Cov(M^0_i + M^1_i, M^0_j + M^1_j) \\
    &= \frac{1}{4} \Big( \Cov(M^0_i, M^0_j) + \Cov(M^1_i, \bar M^1_j) + \Cov(M^0_i, M^1_j) + \Cov(M^1_i, M^0_j) \Big) \\
    &= \frac{1}{2} \Big( \Cov(M^0_i, M^0_j) + \Cov(M^0_i, M^1_j) \Big).
\end{align*}

We can now compare $\Sigma_{\bar b}$ to $\Sigma_{\check b}$. To account for each $\bar M$ sample requiring twice as many cooperative game evaluations as $M^0$, we compare the covariance $\Cov(\bar b_{2n})$ to the covariance $\Cov(\check b_n)$:
% when we compare the covariance of $b_{2n}$ and $\check b_n$, we get the following result:

\begin{align*}
    n \Big(\Cov(\bar b_{2n}) - \Cov(\check b_n) \Big)_{ij} &= - \frac{1}{2} \Cov(M^0_i, M^1_j).
    % &= - \frac{1}{2} \Cov \Big(Z_i \big( v(Z) - v(\mathbf{0}) \big), (1 - Z_i) \big( v(\mathbf{1} - Z) - v(\mathbf{0}) \big) \Big).
\end{align*}

Based on this, we define $G_v$ as follows:

\begin{align*}
    G_v &= - \Cov(M^0_i, M^1_j) \\
    % &= - \Cov \Big(Z_i \big( v(Z) - v(\mathbf{0}) \big), (1 - Z_i) \big( v(\mathbf{1} - Z) - v(\mathbf{0}) \big) \Big). \\
    &= - \Cov\Big(Zv(Z) - \E[Z]v(\mathbf{0}), (\mathbf{1} - Z)v(\mathbf{1} - Z) - \E[\mathbf{1} - Z]v(\mathbf{0})\Big) \\
    &= - \Cov\Big(Zv(Z), (\mathbf{1} - Z)v(\mathbf{1} - Z)\Big).
\end{align*}

This is the matrix referenced in Theorem~\ref{thm:confidence}. Notice that $G_v$ is the negated cross-covariance between $M^0$ and $M^1$, which is the off-diagonal block in the joint covariance matrix for the concatenated random variable $(M^0, M^1)$. This matrix is symmetric, unlike general cross-covariance matrices, and its eigen-structure determines whether our variance reduction approach is effective. In particular, if the condition $G_v \succeq 0$ is satisfied, then we have

\begin{align*}
    \Cov(\bar b_{2n}) \succeq \Cov(\check b_n),
\end{align*}

which implies that

\begin{align*}
    \Cov(\bar \beta_{2n}) \succeq \Cov(\check \beta_n).
\end{align*}

Since the inverses of two ordered matrices are also ordered, we get the result:

\begin{align*}
    \Cov(\bar \beta_{2n})\inv \preceq \Cov(\check \beta_n)\inv.
\end{align*}

This has implications for quadratic forms involving each matrix. For any vector $a \in \R^d$, we have the inequality

\begin{align*}
    a^T\Cov(\bar \beta_{2n})\inv a \leq a^T\Cov(\check \beta_n)\inv a.
\end{align*}

The last inequality has a geometric interpretation. It shows that the confidence ellipsoid (i.e., the confidence region, or prediction ellipsoid) for $\check \beta_n$ is contained by the corresponding confidence ellipsoid for $\bar \beta_{2n}$ since large values of $n$ lead each estimator to converge to its asymptotically normal distribution. This is because the confidence ellipsoids are defined for $\alpha \in (0, 1)$ as

\begin{align*}
    & \bar E_{2n, \alpha} = \Big\{a \in \R^d: (a - \beta^*)^T \Cov(\bar \beta_{2n})\inv (a - \beta^*) \leq \sqrt{\chi^2_d(\alpha)} \Big\} \\
    & \check E_{n, \alpha} = \Big\{a \in \R^d: (a - \beta^*)^T \Cov(\check \beta_{n})\inv (a - \beta^*) \leq \sqrt{\chi^2_d(\alpha)} \Big\},
\end{align*}

where $\chi^2_d(\alpha)$ denotes the inverse CDF of a Chi-squared distribution with $d$ degrees of freedom evaluated at $\alpha$. More precisely, we have $\check E_{n, \alpha} \subseteq \bar E_{2n, \alpha}$ because

\begin{align*}
    &(a - \beta^*)^T \Cov(\check \beta_{n})\inv (a - \beta^*) \leq \sqrt{\chi^2_d(\alpha)} \\
    \Rightarrow &(a - \beta^*)^T \Cov(\bar \beta_{2n})\inv (a - \beta^*) \leq \sqrt{\chi^2_d(\alpha)}.
\end{align*}

This completes the proof.

% Return to this later when trying to prove that $G_v \succeq 0$ for all v
% Schur product property: https://en.wikipedia.org/wiki/Definite_symmetric_matrix#Hadamard_product
% Diagonal dominance probably won't help: https://en.wikipedia.org/wiki/Diagonally_dominant_matrix#Applications_and_properties

\subsection{A Weaker Condition}

Consider the matrix $G_v$, which for a game $v$ is defined as

\begin{equation*}
    G_v = - \Cov\Big(Zv(Z), (\mathbf{1} - Z)v(\mathbf{1} - Z)\Big).
\end{equation*}

A necessary (but not sufficient) condition for $G_v \succeq 0$ is that its diagonal elements are non-negative. We can prove that this weaker condition holds for all games. For an arbitrary game $v$, the diagonal value $(G_v)_{ii}$ is given by:

\begin{align*}
    (G_v)_{ii} &= - \Cov\Big(Z_i v(Z), (1 - Z_i) v(\mathbf{1} - Z)\Big) \\
    &= - \E\big[Z_i(1 - Z_i)v(Z)v(\mathbf{1} - Z)\big] + \E\big[Z_iv(Z)\big]\E\big[(1 - Z_i)v(\mathbf{1} - Z)\big] \\
    &= \E\big[Z_iv(Z)\big]^2 \\
    &= \E\big[v(S) | i \in S\big]^2 \\
    &\geq 0.
\end{align*}

Geometrically, this condition means that the confidence ellipsoid $\bar E_{2n, \alpha}$ extends beyond the ellipsoid $\check E_{n, \alpha}$ in the axis-aligned directions. In a probabilistic sense, it means that the variance for each Shapley value estimate is lower when using the paired sampling technique.

\section{SHAPLEY EFFECTS} \label{app:shapley_effects}

Shapley Effects is a model explanation method that summarizes the model $f$'s sensitivity to each feature \cite{owen2014sobol}. It is based on the cooperative game

\begin{equation}
     \tilde w(S) = \Var\big(\E[f(X) | X_S]\big).
\end{equation}

To show that Shapley Effects can be viewed as the expectation of a stochastic cooperative game, we  reformulate this game (Covert et al. \cite{covert2020understanding}) as:

\begin{align*}
    \tilde w(S) &= \Var\big(\E[f(X) | X_S]\big) \\
    &= \Var\big(f(X)\big) - \E_{X_S}\big[\Var(f(X) | X_S)\big] \\
    &= c - \E_{X_S} \Big[ \E_{X_{D \setminus S} | X_S}\big[\big(\E[f(X) | X_S] - f(X_S, X_{D \setminus S}) \big)^2 \big] \Big] \\
    &= c - \E_X \Big[ \big( \E[f(X) | X_S] - f(X) \big)^2 \Big].
\end{align*}

If we generalize this cooperative game to allow arbitrary loss functions (e.g., cross entropy loss for classification tasks) rather than MSE, then we can ignore the constant value and re-write the game as

\begin{align*}
    \tilde w(S) = - \E_X\Big[ \ell\big(\E[f(X) | X_S], f(X)\big)\Big].
\end{align*}

Now, it is apparent that Shapley Effects is based on a cooperative game that is the expectation of a stochastic cooperative game, or $\tilde w(S) = \E_X[\tilde W(S, X)]$, where $\tilde W(S, X)$ is defined as:

\begin{equation*}
    \tilde W(S, X) = - \ell \big( \E[f(X) | X_S], f(X) \big).
\end{equation*}

Unlike the stochastic cooperative game implicitly used by SAGE, the exogenous random variable for this game is $U = X$.

\section{STOCHASTIC COOPERATIVE GAME PROOFS} \label{app:stochastic}

% \textcolor{blue}{There was a mistake in the main text and we apologize to the reviewers for the confusion. Both the original and unbiased versions of KernelSHAP can be adapted to the setting of stochastic cooperative games to provide consistent Shapley value estimators. This section describes how both of these approaches work, correcting our mistake in the main text.}

For a stochastic cooperative game $V(S, U)$, the generalized Shapley values are given by the expression

\begin{align*}
    \phi_i(V) &= \frac{1}{d} {\sum_{S {\subseteq} D {\setminus} \{i\}}} \binom{d {-} 1}{|S|}^{{-}1} \E_U\big[ V(S \cup \{i\}, U) {-} V(S, U) \big] \\
    &= \frac{1}{d} {\sum_{S {\subseteq} D {\setminus} \{i\}}} \binom{d {-} 1}{|S|}^{{-}1} \E_U\big[ V(S \cup \{i\}, U) \big] - \E_U\big[V(S, U) \big].
\end{align*}

The second line above shows that the generalized Shapley values are equivalent to the Shapley values of the game's expectation, or $\phi_i(\bar V)$, where $\bar V(S) = \E_U[V(S, U)]$. Based on this, we can also understand the values $\phi_1(V), \ldots, \phi_d(V)$ as the optimal coefficients for the following weighted least squares problem:

\begin{align*}
    &\min_{\beta_0, \ldots, \beta_d} \; \sum_z p(z) \Big(\beta_0 + z^T \beta - \E_U\big[V(z, U)\big] \Big)^2 \nonumber \\
    &\mathrm{s.t.} \quad \beta_0 = \E_U\big[V(\mathbf{0}, U) \big], \quad \mathbf{1}^T \beta = \E_U\big[V(\mathbf{1}, U) \big] - \E_U\big[V(\mathbf{0}, U) \big].
\end{align*}

Using our derivation from the main text (Section~\ref{sec:exact}),
% (Section~3.3),
we can write the solution as

\begin{equation*}
    \beta^* = A\inv \Big(b - \mathbf{1} \frac{\mathbf{1}^T A\inv b - \E_U[V(\mathbf{1}, U) ] + \E_U[V(\mathbf{0}, U) ]}{\mathbf{1}^T A\inv \mathbf{1}}\Big),
\end{equation*}

where $A$ and $b$ are given by the expressions

\begin{align*}
    A &= \E[ZZ^T] \\
    b &= \E_Z\Big[Z \big(\E_U[V(Z, U) ] - \E_U[V(\mathbf{0}, U) ]\big)\Big]. % \\
    % &= \E_{ZU} \Big[Z \big(V(Z, U) - \E_U[V(\mathbf{0}, U) ]\big)\Big] \\
    % &= \E_{ZU} \big[Z V(Z, U) \big] - \E_Z\big[Z\big] \E_U\big[V(\mathbf{0}, U) \big] \\ % This is what stochastic does
    % &= \E_{ZU} \Big[Z \big(V(Z, U) - V(\mathbf{0}, U) \big)\Big] % This is what KernelSHAP does
\end{align*}

Now, we consider our adaptations of KernelSHAP and unbiased KernelSHAP and examine whether these estimators are consistent or unbiased. We begin with the stochastic version of KernelSHAP presented in the main text (Section~\ref{sec:stochastic_kernelshap}). Recall that this approach uses the original $A$ estimator $\hat A_n$ and the modified $b$ estimator $\tilde b_n$, which is defined as:

\begin{equation*}
    \tilde b_n = \frac{1}{2} \sum_{i = 1}^n z_i \big( V(z_i, u_i) - \E_U\big[V(\mathbf{0}, U)\big] \big).
\end{equation*}

As mentioned in the main text, the strong law of large numbers lets us conclude that $\lim_{n \to \infty} \hat A_n = A$. Thus, we can understand the $b$ estimator's expectation as follows:

\begin{align*}
    \E\big[ \tilde b_n \big] &= \E_{ZU} \Big[ Z \big( V(Z, U) - \E_U\big[V(\mathbf{0}, U)\big] \big) \Big] \\
    &= \E_Z\Big[Z \big(\E_U[V(Z, U) ] - \E_U[V(\mathbf{0}, U) ]\big)\Big] \\
    &= b.
\end{align*}

With this, we conclude that $\lim_{n \to \infty} \tilde b_n = b$ and that $\tilde \beta_n$ are consistent, or

\begin{equation*}
    \lim_{n \to \infty} \tilde \beta_n = \beta^*.
\end{equation*}

To adapt unbiased KernelSHAP to the setting of stochastic cooperative games, we use the same technique of pairing independent samples of $Z$ and $U$.
% With abuse of notation, we re-use symbols used to denote estimators for the stochastic version of KernelSHAP.
To estimate $b$, we use an estimator $\tilde{\bar b}_n$ defined as:

\begin{equation*}
    \tilde{\bar b}_n = \frac{1}{n} \sum_{i = 1}^n z_iV(z_i, u_i) - \E\big[Z\big]\E_U\big[V(\mathbf{0}, U)\big].
\end{equation*}

We then substitute this into a Shapley value estimator as follows:

\begin{equation}
     \tilde{\bar \beta}_n = A\inv \Big(\tilde{\bar b}_n - \mathbf{1} \frac{\mathbf{1}^T A\inv \tilde{\bar b}_n - v(\mathbf{1}) + v(\mathbf{0})}{\mathbf{1}^T A\inv \mathbf{1}}\Big).
\end{equation}

This is consistent and unbiased because of the linear dependence on $\tilde{\bar b}_n$ and the fact that $\tilde{\bar b}_n$ is unbiased:
% an unbiased estimator of $b$:

\begin{align*}
    \E\big[ \tilde{\bar b}_n \big] &= \E_{ZU} \Big[ ZV(Z, U) - \E\big[Z\big]\E_U\big[V(\mathbf{0}, U)\big] \Big] \\
    &= \E_Z\Big[Z \big(\E_U[V(Z, U) ] - \E_U[V(\mathbf{0}, U) ]\big)\Big] \\
    &= b.
\end{align*}

With this, we conclude that $\E[\tilde{\bar \beta}_n] = \beta^*$ and $\lim_{n \to \infty} \tilde{\bar \beta}_n = \beta^*$.


% When estimating the solution using unbiased KernelSHAP, we use the estimator $\tilde \beta_n$ defined as

% \begin{align*}
%     \tilde \beta_n = A\inv \Big(\tilde b_n - \mathbf{1} \frac{\mathbf{1}^T A\inv \tilde b_n - \E_U[V(\mathbf{1}, U) ] + \E_U[V(\mathbf{0}, U) ]}{\mathbf{1}^T A\inv \mathbf{1}}\Big),
% \end{align*}

% where $\tilde b_n$ uses $n$ samples $z_i \sim p(Z)$ and is given by

% \begin{align*}
%     \tilde b_n = \frac{1}{n} \sum_{i = 1}^n z_iV(z_i, u_i) - \E[Z]\E_U[V(\mathbf{0}, U)].
% \end{align*}

% We can see that this estimator is both consistent and unbiased because of $\tilde b_n$'s expectation:

% \begin{align*}
%     \E\big[\tilde b_n\big] &= \E_{ZU} \big[ZV(Z, U) \big] - \E\big[Z\big]\E_U\big[V(\mathbf{0}, U)\big] \\
%     &= \E_Z \big[ Z \E_U[V(Z, U)] \big] - \E[Z]\E_U[V(\mathbf{0}, U)] \\
%     &= b.
% \end{align*}

% The estimator remains consistent and unbiased when we incorporate the variance reduction technique described in Section~4.2.





% \textcolor{red}{By looking at the optimization problem, we can imagine several ways of sampling pairs $z_i, u_i$ to approximate the objective. There are least three estimators to compare, depending on the extent to which they use an expectation over $U$. Jensen's inequality seems to suggest that the approximate objective upper bounds an approximate version of the true objective; given that the solutions optimize the wrong objective, it seems that they won't be consistent. However, they all appear to be consistent when we look at $\hat b$'s expectation.}

% \textcolor{red}{With this, I think I've shown that KernelSHAP does yield a consistent estimator. If the variance decreases at a rate of $\frac{1}{n}$, it's possible that this is preferable to the unbiased version, if its variance goes down faster.}

% \textcolor{red}{Unfortunately, the only way to sort out these questions is by running the estimators to convergence many times...}

% TODO getting random here

% Here's what the KernelSHAP estimator does:

% \begin{align*}
%     \hat b_n &= \frac{1}{n} \sum_{i = 1}^n z_i \Big(V(z_i, u_i) - V(\mathbf{0}, u_i)\Big) \\
%     \hat b_n &= \frac{1}{n} \sum_{i = 1}^n z_i \Big(V(z_i, u_i) - \E_U[V(\mathbf{0}, U)] \Big)
% \end{align*}

% Here's what the KernelSHAP estimator would look like if it used the game's expectation (in which case it's definitely consistent):

% \begin{align*}
%     \hat b_n &= \frac{1}{n} \sum_{i = 1}^n z_i \Big(\E[V(z_i, U)] - \E_U[V(\mathbf{0}, U)]\Big) \\
%     &\to \E_Z \Big[ Z \Big(\E[V(Z, U)] - \E_U[V(\mathbf{0}, U)]\Big) \Big] \\
%     &= b.
% \end{align*}

% God damn it, the KernelSHAP estimator appears to be consistent whether it uses the game's expectation or not. How is that possible? The two estimators are based on two unequal objectives. Jensen's says that one upper bounds the other, and they're definitely not the same. What am I missing?

% \section{ALGORITHM FOR STOCHASTIC COOPERATIVE GAMES}

% Algorithm~\ref{alg:stochastic} provides the pseudocode for our linear regression-based approach to estimating the generalized Shapley values of stochastic cooperative games. It is a slight modification of Algorithm~1, see Section~5.3 of the main text for more details.

% % \addtocounter{algocf}{1}
% \input{algorithm_stochastic}

\section{EXPERIMENT DETAILS} \label{app:experiments}

Here, we provide further details about experiments described in the main body of text.

\subsection{Datasets and Hyperparameters}

For all three explanation methods considered in our experiments -- SHAP \cite{lundberg2017unified}, SAGE \cite{covert2020understanding} and Shapley Effects \cite{owen2014sobol} -- we handled removed features by marginalizing them out according to their joint marginal distribution. This is the default behavior for SHAP, but it is an approximation of what is required by SAGE and Shapley Effects. However, this choice should not affect the outcome of our experiments, which focus on the convergence properties of our Shapley value estimators (and not the underlying cooperative games).

Both SAGE and Shapley Effects require a loss function (Section~\ref{app:shapley_effects}). We used the cross entropy loss for SAGE and the soft cross entropy loss for Shapley Effects.

For the breast cancer (BRCA) subtype classification dataset, we selected 100 out of 17,814 genes to avoid overfitting on the relatively small dataset size (only 510 patients). These genes were selected at random: we tried ten random seeds and selected the subset that achieved the best performance to ensure that several relevant BRCA genes were included. A small portion of missing expression values were imputed with their mean. The data was centered and normalized prior to fitting a $\ell_1$ regularized logistic regression model; the regularization parameter was chosen using a validation set.

% For the BRCA dataset, we randomly selected a subset of 100 genes to analyze out of 17,814 total. To ensure that a sufficient number BRCA-associated genes were selected, we tried 10 random seeds for the gene selection step and selected the seed whose 100 genes achieved the best performance. The selected genes are shown in Table~\ref{tab:genes}. A small portion of missing expression values were imputed with their mean. The data was centered and normalized prior to fitting the regularized logistic regression model.

% \textcolor{purple}{Used marginal distribution for all methods; not important to estimator properties. Take text from explaining by removing to describe gene selection. Model hyperparameters chosen using separate validation set; also not important to estimator properties. Used cross entropy loss for SAGE and soft cross entropy loss for Shapley Effects.}

\subsection{SHAP Run-time Comparison}

To compare the run-time of various SHAP value estimators, we sought to compare the ratio of the mean number of samples required by each method. For a single example $x$ whose SHAP values are represented by $\beta^*$, the mean squared estimation error can be decomposed into the variance and bias as follows:

\begin{equation*}
    \E\big[||\hat \beta_n - \beta^*||^2\big] = \E\big[||\hat \beta_n - \E[\hat \beta_n]||^2\big] + \big|\big|\E[\hat \beta_n] - \beta^*\big|\big|^2.
\end{equation*}

Since we found that the error is dominated by variance rather than bias (Section~\ref{sec:properties}), we can make the following approximation to relate the error to the trace of the covariance matrix:

\begin{align}
    \E\big[||\hat \beta_n - \beta^*||^2\big] &= \E\big[||\hat \beta_n - \E[\hat \beta_n]||^2\big] + \big|\big|\E[\hat \beta_n] - \beta^*\big|\big|^2 \nonumber \\
    &\approx \E\big[||\hat \beta_n - \E[\hat \beta_n]||^2\big] \nonumber \\
    % &= \Tr\Big( \E\big[(\hat \beta_n - \E[\hat \beta_n])(\hat \beta_n - \E[\hat \beta_n])^T\big] \Big) \\
    &= \Tr\Big( \Cov(\hat \beta_n) \Big). \label{eq:error_approximation}
\end{align}

If we define convergence based on the mean estimation error falling below a threshold value $t$, then the convergence condition is

\begin{equation*}
    \E\big[||\hat \beta_n - \beta^*||^2\big] \leq t.
\end{equation*}

Using our approximation (Eq.~\ref{eq:error_approximation}), we can see that this condition is approximately equivalent to

\begin{equation*}
    \E\big[||\hat \beta_n - \beta^*||^2\big] \approx \Tr\Big( \Cov(\hat \beta_n) \Big) \approx \frac{\Tr(\Sigma_{\hat \beta})}{n} \leq t.
\end{equation*}

For a given threshold $t$, the mean number of samples required to explain individual predictions is therefore based on the mean trace of the covariance matrix $\Sigma_{\hat \beta}$ (or the analogous covariance matrix for a different estimator). To compare two methods, we simply calculate the ratio of the mean trace of the covariance matrices. These ratios are reported in Table~\ref{tab:shap_comparison}, where each covariance matrix is calculated empirically across 100 runs with $n = 2048$ samples.

\section{CONVERGENCE EXPERIMENTS} \label{app:convergence_experiments}

In Section~\ref{sec:properties}, we empirically compared the bias and variance for the original and unbiased versions of KernelSHAP using a single census income prediction. The results (Figure~\ref{fig:error}) showed that both versions' estimation errors were dominated by variance rather than bias, and that the original version had significantly lower variance. To verify that this result is not an anomaly, we replicated it on multiple examples and across several datasets.

First, we examined several individual predictions for the census income, German credit and bank marketing datasets. To highlight the effectiveness of our paired sampling approach (Section~\ref{sec:var_reduction}), we added these methods as additional comparisons. Rather than decomposing the error into bias and variance as in the main text, we simply calculated the mean squared error across 100 runs of each estimator. Figure~\ref{fig:census_mse} shows the error for several census income predictions, Figure~\ref{fig:bank_mse} for several bank marketing predictions, and Figure~\ref{fig:credit_mse} for several credit quality predictions. These results confirm that the original version of KernelSHAP converges significantly faster than the unbiased version, and that the paired sampling technique is effective for both estimators. The dataset sampling approach (original KernelSHAP) appears preferable in practice despite being more difficult to analyze because it converges to the correct result much faster.

Second, we calculated a global measure of the bias and variance for each estimator using the same datasets (Table~\ref{tab:bias_variance}). Given 100 examples from each dataset, we calculated the mean bias and mean variance for each estimator empirically across 100 runs given $n = 256$
% 2048
samples. Results show that the bias is nearly zero for all estimators, not just the unbiased ones; they also show that the variance is often significantly larger than the bias. However, when using the dataset sampling approach (original) in combination with the paired sampling technique, the bias and variance are comparably low ($\approx 0$) after 256
% 2048
samples. The only exception is the unbiased estimator that does not use paired sampling, but this is likely due to estimation error because its bias is provably equal to zero.

Finally, Section~\ref{sec:convergence} also proposed assuming that the original KernelSHAP estimator's variance reduces at a rate of $\mathcal{O}(\frac{1}{n})$, similar to the unbiased version (for which we proved this rate). Although this result is difficult to prove formally, it seems to hold empirically across multiple predictions and several datasets. In Figures~\ref{fig:census_variance}, ~\ref{fig:bank_variance} and ~\ref{fig:credit_variance}, we display the product of the estimator's variance with the number of samples for the census, bank and credit datasets. Results confirm that the product is roughly constant as the number of samples increases, indicating that the variance for all four estimators (not just the unbiased ones) reduces at a rate of $\mathcal{O}(\frac{1}{n})$.

\input{inserts/bias-variance}

\input{inserts/census_mse}
\input{inserts/bank_mse}
\input{inserts/credit_mse}

\section{ALGORITHMS} \label{app:algorithms}

Here, we provide pseudocode for the estimation algorithms described in the main text. Algorithm~\ref{alg:kernelshap} shows the dataset sampling approach (original KernelSHAP) with our convergence detection and paired sampling techniques. Algorithm~\ref{alg:kernelshap_stochastic} shows KernelSHAP's adaptation to the setting of stochastic cooperative games (stochastic KernelSHAP). Algorithm~\ref{alg:unbiased} shows the unbiased KernelSHAP estimator, and Algorithm~\ref{alg:unbiased_stochastic} shows the adaptation of unbiased KernelSHAP to stochastic cooperative games.

\input{algorithms/kernelshap}
\input{algorithms/kernelshap_stochastic}
\input{algorithms/unbiased}
\input{algorithms/unbiased_stochastic}


==> old/body.tex <==
\section{Introduction}

KernelSHAP is one of the most popular methods for estimating SHAP values, which are the Shapley values of a cooperative game representing an individual prediction. The method is based on Scott's observation that Shapley values are the solution to a weighted constrained linear regression problem.

Despite KernelSHAP's popularity, I expect that many people don't understand how it works. I'm one of those people. But I need to understand it to implement it for my Shapley value estimation implementations (particularly SAGE). In these notes, I'll derive how to estimate a cooperative game's Shapley values by solving a constrained least squares problem.

\section{Linear Regression}

A linear regression model with data points $(x_i, y_i)$ for $i = 1, 2, \ldots, n$ is fit by solving the following least squares problem:

\begin{align*}
    \sum_{i=1}^n (x-i^T \beta + \beta_0 - y_i)
    &= ||X\beta + \mathbf{1}\beta_0 - Y||^2 \\
    &= ||\begin{pmatrix}\mathbf{1} & X \end{pmatrix} \begin{pmatrix} \beta_0 \\ \beta \end{pmatrix} - Y||^2
\end{align*}

A weighted least squares problem is given by the following:

\begin{align*}
    \Big(\begin{pmatrix}\mathbf{1} & X \end{pmatrix} \begin{pmatrix} \beta_0 \\ \beta \end{pmatrix} - Y\Big)^T W \Big(\begin{pmatrix}\mathbf{1} & X \end{pmatrix} \begin{pmatrix} \beta_0 \\ \beta \end{pmatrix} - Y\Big)
\end{align*}

where $W$ is a diagonal matrix with entries specifying the weights for each data point.

Shapley values are based on solving a weighted least squares problem, with weights given by the ``Shapley kernel,'' as it is informally known. However, we won't be able to solve it as a weighted least squares problem because we can't obtain all the necessary data points. Instead, we'll re-express the objective as an expectation over a distribution.

\begin{align*}
    \sum_{i = 1}^n w_i (x_i^T \beta + \beta_0 - y_i)^2
    &= \E[(X^T \beta + \beta_0 - Y)]
\end{align*}

In the above, capital letters refer to random variables rather than matrices (as in the linear algebra equations further above). Now, we can estimate this objective by sampling $x$ according to the distribution induces by the weights $w_i$.

\begin{align*}
    \E[(X^T \beta + \beta_0 - Y)]
    &\approx \frac{1}{n} \sum_{i = 1}^n (x_i^T \beta + \beta_0 - y_i)^2 \\
    &= \frac{1}{n} ||\begin{pmatrix}\mathbf{1} & X \end{pmatrix} \begin{pmatrix} \beta_0 \\ \beta \end{pmatrix} - Y||^2
\end{align*}

where $X, Y$ are now matrices containing the samples $x_i, y_i$. This can be understood as a stochastic estimator of the true objective. If we expand it we can see that it's consistent:

\begin{align*}
    \frac{1}{n} \Big(\begin{pmatrix} \beta_0 \\ \beta \end{pmatrix}^T \begin{pmatrix}\mathbf{1} & X \end{pmatrix}^T \begin{pmatrix}\mathbf{1} & X \end{pmatrix} \begin{pmatrix} \beta_0 \\ \beta \end{pmatrix}
    - 2 Y^T \begin{pmatrix}\mathbf{1} & X \end{pmatrix} \begin{pmatrix} \beta_0 \\ \beta \end{pmatrix}
    + Y^TY \Big)
\end{align*}

It's consistent because the two variance and the one covariance term are consistent estimators. It's not quite unbiased, but I think it could be made unbiased with a simple modification of $\frac{1}{n}$ to $\frac{1}{n - 1}$. This isn't important, we're not as focused on our estimator of the objective as we are on the problem's solution.

Solving this problem is pretty easy when we use matrix derivatives. But unfortunately, the Shapley problem is even more complicated than this because it incorporates constraints.

When Shapley values are expressed as the solution to a weighted least squares problem, it has two constraints:

\begin{align*}
    \beta_0 &= v(\varnothing) \\
    \sum_{i = 1}^d \beta_i &= v(D) - v(\varnothing)
\end{align*}

In our case, if we sample data points according to some distribution that matches the Shapley kernel conditioned on points being included, then we can simply partition our samples into three sets: 1) those where all features are included, 2) those where no features are included, 3) those where some features are included. Then we can use this to estimate constants corresponding to the constraints. TODO come back to this

The Shapley kernel is the following:

\begin{align*}
    \pi(S) = \frac{d - 1}{\binom{d}{|S|}|S|(d - |S|)}
\end{align*}

Now, for $S$ such that $0 < |S| < d$ (the prediction is not fixed by constraints), we have:

\begin{align*}
    \pi(S) &= \frac{(|S| - 1)!(d - |S| - 1)!}{(d - 1)!} \\
    &= \frac{1}{d - 1} \binom{d - 2}{|S| - 1}\inv
\end{align*}

This is consistent with the kernel described by Charnes at al., at least according to Hammer and Holtzman (since I can't access the Charnes paper). Now, I must figure out how to sample from a distribution that's close to this.

\clearpage

\section{Regression-Based Estimates for Shapley Values}

Here's an easier way to think about this. We have a cooperative game $v: \mathcal{P}(D) \mapsto \R$, and with abuse of notation we can think of this as a function $v: \{0, 1\}^d \mapsto \R$. The input coalitions $S \subseteq D$ can be represented as binary vectors $x \in \{0, 1\}^d$, and we can imagine fitting a weighted linear model as follows:

\begin{align*}
    \sum_{x} w(x) \big(\beta_0 + \sum_{i = 1}^d x_i \beta_i - v(x)\big)^2
\end{align*}

The Shapley value can be expressed as a solution to one of these problems, but with a kernel that effectively puts constraints on $\beta_0, \ldots, \beta_d$. The problem looks like the following:

\begin{align*}
    &\sum_{x} \pi(x) \big(\beta_0 + \sum_{i=1}^d x_i \beta_i - v(c) \big) \\
    &\mathrm{s.t.} \quad \beta_0 = v(\{\}), \quad \sum_{i = 1}^d \beta_i = v(D) - v(\{\})
\end{align*}

where the weighting kernel is given by

\begin{align*}
    \pi(x) = \begin{cases}
        \binom{d-2}{|S| - 1}\inv \quad\quad 0 < \mathbf{1}^Tx < d \\
        0 \quad\quad \mathrm{else}
    \end{cases}
\end{align*}

For large values of $d$, we won't be able to calculate this full objective or obtain the closed-form solution. Instead, we find the exact solution to an approximate version of the objective, and sample $x$'s according to the distribution induced by $\pi$. Our approximate objective is:

\begin{align*}
    &\frac{1}{n} \sum_{i = 1}^n \big(\beta_0 + \sum_{j = 1}^d x_{ij} \beta_j - v(x_i) \big)^2 \\
    &\mathrm{s.t.} \quad \beta_0 = v(\{\}), \quad \sum_{i = 1}^d \beta_i = v(D) - v(\{\})
\end{align*}

Solving this problem is much more manageable. We rewrite it by denoting $\beta = (\beta_1, \ldots, \beta_d)$ and using matrix notation:

\begin{align*}
    &\frac{1}{n} ||X \beta - (Y - \mathbf{1} \beta_0)||^2 \\
    &\mathrm{s.t.} \quad \beta_0 = v(\{\}), \quad \sum_{i = 1}^d \beta_i = v(D) - v(\{\})
\end{align*}

where $Y_i = v(x_i)$. We can find a closed form solution to this problem by solving the Lagrangian:

\begin{align*}
    \mathcal{L}(\beta, \lambda) &= \frac{1}{n}||X \beta - (Y - \mathbf{1} \beta_0)||^2 + 2 \lambda (\mathbf{1}^T \beta - v(D) + v(\{\}))
\end{align*}

If we take the derivative with respect to $\beta$ we get:

\begin{align*}
    \frac{\partial \mathcal{L}}{\partial \beta}(\beta, \lambda) = 2 \big(\frac{1}{n} X^TX\big) \beta - 2 \Big(\frac{1}{n}X^T \big(Y - \mathbf{1}v(\{\})\big) \Big) + 2 \mathbf{1}\lambda
\end{align*}

This yields the closed-form solution:

\begin{align*}
    \beta^* = \big(\frac{1}{n} X^TX\big)\inv \Big(\frac{1}{n} X^T \big(Y - \mathbf{1}v(\{\})\big) - \mathbf{1}\lambda \Big)
\end{align*}

The only remaining question is, what value does the dual variable $\lambda$ take for the optimal solution? We can find this by using the fact that the constraint must hold:

\begin{align*}
    \mathbf{1}^T \beta^* = v(D) - v(\{\})
\end{align*}

This gives us the following equation for $\lambda$:

\begin{align*}
    \lambda = \Big[\mathbf{1}^T \big(\frac{1}{n} X^TX\big)\inv (\frac{1}{n} X^T \big(Y - \mathbf{1}v(\{\})\big) - \big(v(D) - v(\{\})\big) \Big] / \Big(\mathbf{1}^T \big(\frac{1}{n} X^TX\big)\inv \mathbf{1}\Big)
\end{align*}

And finally, this gives us the following solution for $\beta^*$:

\begin{align*}
    \beta^* = \; &\big(\frac{1}{n} X^TX\big)\inv \frac{1}{n} X^T \big(Y - \mathbf{1}v(\{\})\big) \\
    &- \Big(\mathbf{1}^T \big(\frac{1}{n} X^TX\big)\inv \mathbf{1}\Big)\inv \big(\frac{1}{n} X^TX\big)\inv \mathbf{1}\Big(\mathbf{1}^T \big(\frac{1}{n} X^TX\big)\inv (\frac{1}{n} X^T \big(Y - \mathbf{1}v(\{\})\big) - \big(v(D) - v(\{\})\big) \Big)
\end{align*}

We can simplify this by denoting the following quantities:

\begin{align*}
    A &= \frac{1}{n}X^TX \\
    b &= \frac{1}{n} X^TY \\
    c &= \frac{1}{n} X^T \mathbf{1} \\
    a_0 &= v(\{\}) \\
    a_1 &= v(D) - v(\{\})
\end{align*}

This allows us to rewrite the solution as:

\begin{align*}
    \beta^* = A\inv (b - ca_0) - (\mathbf{1}^T A\inv \mathbf{1})\inv A\inv \mathbf{1} \Big(\mathbf{1}^T A\inv (b - ca_0) - a_1\Big)
\end{align*}

We can remove certain sources of stochasticity from this estimator by using the exact form for a couple of these terms. In particular, the following quantities can be calculated exactly using the distribution induced by $\pi$:

\begin{align*}
    \E[A_{ij}] &= p(i, j \in S) \\
    \E[c_i] &= p(i \in S)
\end{align*}

These can be calculated exactly, but they require us to consider the distribution over subsets more carefully. The distribution induced by $\pi$ for $S$ such that $0 < |S| < d$ is

\begin{align*}
    p(S) = \alpha \binom{d - 2}{|S| - 1}\inv
\end{align*}

which means that $\alpha$ is given by

\begin{align*}
    \alpha\inv &= \sum_{0 < |S| < d} \binom{d - 2}{|S| - 1}\inv \\
    &= \sum_{k = 1}^{d - 1} \binom{d}{k} \binom{d - 2}{k - 1}\inv \\
    &= \sum_{k = 1}^{d - 1} \frac{d!}{k!(d-k)!} \frac{(k-1)!(d-k-1)!}{(d-2)!} \\
    &= \sum_{k=1}^{d-1} \frac{d(d-1)}{k(d-k)}
\end{align*}

Now, we can see that the exact values for $\E[c]$ is given by:

\begin{align*}
    \E[c_i] &= p(i \in S) \\
    &= \sum_{k = 1}^{d-1} p(i \in S \; | \; |S| = k) p(|S| = k) \\
    &= \alpha \sum_{k = 1}^{d-1} \binom{d - 1}{k - 1}\binom{d}{k}\inv \cdot \binom{d}{k} \binom{d - 2}{k - 1}\inv \\
    &= \alpha \sum_{k = 1}^{d - 1} \frac{d - 1}{d - k} \\
    &= \frac{\sum_{k = 1}^{d - 1} \frac{d - 1}{d - k}}{\sum_{k=1}^{d-1} \frac{d(d-1)}{k(d-k)}}
\end{align*}

We can prove that this is equal to $\frac{1}{2}$ as follows:

\begin{align*}
    1 - \E[c_i] &= 1 - \frac{\sum_{k = 1}^{d - 1} \frac{d - 1}{d - k}}{\sum_{k=1}^{d-1} \frac{d(d-1)}{k(d-k)}} \\
    &= \Big( \sum_{k=1}^{d-1} \frac{d(d-1)}{k(d-k)} \Big)\inv \Big(\sum_{k=1}^{d-1} \frac{d(d-1)}{k(d-k)} - \sum_{k = 1}^{d - 1} \frac{d - 1}{d - k} \Big) \\
    &= \Big( \sum_{k=1}^{d-1} \frac{d(d-1)}{k(d-k)} \Big)\inv \Big(\sum_{k=1}^{d-1} \frac{d(d-1)}{k(d-k)} - \frac{k(d - 1)}{k(d - k)} \Big) \\
    &= \frac{\sum_{k = 1}^{d - 1} \frac{d - 1}{d - k}}{\sum_{k=1}^{d-1} \frac{d(d-1)}{k(d-k)}} \\
    &= \E[c_i] \\
    &\Rightarrow \E[c_i] = \frac{1}{2}
\end{align*}

Now, we can do a similar analysis for $\E[A_{ij}]$. First, we can see that diagonal entries have the following expectation:

\begin{align*}
    \E[A_{ii}] &= p(i \in S) \\
    &= \E[c_i] \\
    &= \frac{1}{2}
\end{align*}

Off-diagonal entries have the following expectation:

\begin{align*}
    \E[A_{ij}] &= p(i, j \in S) \\
    &= \sum_{k = 2}^{d - 1} p(i, j \in S \; | \; |S| = k) p(|S| = k) \\
    &= \alpha \sum_{k = 2}^{d - 1} \binom{d - 2}{k - 2} \binom{d}{k}\inv \cdot \binom{d}{k} \binom{d - 2}{k - 1}\inv \\
    &= \alpha \sum_{k = 2}^{d - 1} \frac{k - 1}{d - k} \\
    &= \frac{\sum_{k = 2}^{d - 1} \frac{k - 1}{d - k}}{\sum_{k=1}^{d-1} \frac{d(d-1)}{k(d-k)}}
\end{align*}

It doesn't seem like there's a convenient way to simplify this, but we can calculate it numerically for a given value of $d$.

Anyway, this approach shows how to estimate Shapley values by calculating the exact solution to an approximate problem.

\section{An Approximate Solution to the Exact Problem}

Rather than stochastically estimating the objective and then optimizing the approximate objective, let's revisit the true objective:

\begin{align*}
    &\E_{p(S)}\Big[\big(\beta_0 + \sum_{i = 1}^d x_i(S) \beta_i - v(x(S))\big)\Big] \\
    &\mathrm{s.t.} \quad \beta_0 = v(\{\}), \quad \sum_{i = 1}^d \beta_i = v(D) - v(\{\})
\end{align*}

Now, write this using matrix algebra:

\begin{align*}
    % \mathcal{L}(\beta_0, \ldots, \beta_d) &=
    &\; \E_{p(S)}\Big[\big(\beta_0 + \sum_{i = 1}^d x_i(S) \beta_i - v(x(S))\big)\Big] \\
    % &= \E_{p(S)} \Big[ \big(\begin{pmatrix}1 & x \end{pmatrix} \begin{pmatrix} \beta_0 \\ \beta \end{pmatrix} - v(x(S))\big)^2 \Big] \\
    &= \E_{p(S)} \Big[ \big(x^T \beta  - (v(x(S)) - \beta_0)\big)^2 \Big] \\
    &= \E_{p(S)} \Big[ \big(x^T \beta  - (y(x) - \beta_0)\big)^2 \Big] \\
    &= \E_{p(S)} \Big[ \beta^T x x^T \beta - 2 \beta^T x (y(x) - \beta_0) + (y(x) - \beta_0)^2 \Big] \\
    &= \beta^T \E[xx^T] \beta - 2 \beta^T \E[xy(x)] + \E[(y(x) - \beta_0)^2]
\end{align*}

If we use this version of the objective function and write the problem's Lagrangian, we get the following:

\begin{align*}
    \mathcal{L}(\beta, \lambda) = \beta^T \E[xx^T] \beta - 2 \beta^T \E[xy(x)] + \E[(y(x) - \beta_0)^2] + 2\lambda (\mathbf{1}^T \beta - (v(D) - v(\{\})))
\end{align*}

If we solve this, we get the same solution as above, but with $A, b, c$ substituted with their expectations. If we use the exact forms for $\E[A], \E[c]$ and just estimate $b$, then we see how this is an estimator for the solution $\beta^*$ to the true objective.

We can even make a couple remarks about the estimator. The first is that it's consistent, because obviously. The second is that it's unbiased, because the mean is clearly the true value (linear dependence on the only thing being estimated). The third is that the multivariate central limit theorem (MCLT) says that our $b$ estimator asymptotically has a multivariate Gaussian distribution; the estimator therefore asympototically has a multivariate Gaussian distribution. If we estimate $b$'s covariance, then we estimate the estimator's covariance. We use this for providing uncertainty estimates (the diagonal entries) and detecting convergence automatically.

\section{What's Next}

I've found that for SAGE and Shapley Effects, which are for our purposes two stochastic cooperative games, the regression approach has significantly higher variance than the permutation sampling approach. I'm confident in my derivation, and I have empirical evidence that my implementation is correct, so the logical conclusion is that this algorithm simply suffers from higher variance than the permutation sampling algorithm. This was unexpected, because Figure 3 of Scott's NeurIPS paper made it seem like KernelSHAP has way lower variance than IME. 

If Scott was right about KernelSHAP being faster than IME, than maybe I can implement my uncertainty estimates in the removal-based explanations package and see that it 1) gives previously non-existent uncertainty estimates, 2) that it runs faster than the sampling algorithm.

Unfortunately, I haven't really implemented KernelSHAP. I implemented an unregularized constrained least squares problem, but KernelSHAP allows for regularizers. I can get a closed form solution for the ridge version, but not for the Lasso version. What do I do now? I think I need to find an analysis of the variance of a Lasso estimator. These slides are my best hope, they have a shitty variance estimator: \url{http://www.few.vu.nl/~wvanwie/Courses/HighdimensionalDataAnalysis/WNvanWieringen_HDDA_Lecture56_LassoRegression_20182019.pdf}. For $\lambda > 0$ this better yield lower variance than we would get with $\lambda = 0$.

Even if I can figure out how to quantify variance for both types of regularization, I'll have to think about incorporating different weighting kernels (e.g., cosine, uniform). I think that's easy enough: just calculate the weights vector numerically, and then calculate $\E[A]$ and $\E[c]$ numerically.

Then, the last thing to figure out will be how to choose the regularization parameter. For Lasso, people might want to specify the number of non-zero regression coefficients; but what about for Ridge? (That one is interesting to me because it will be easier for me to implement, since closed form solution is almost the same). The usual answer (use cross validation) doesn't work here, because we don't have a validation dataset. In fact, we don't have a dataset at all because I'm only keeping track of sufficient statistics.

I implemented the Ridge penalty and it still didn't fix my problem. It's one thing for the confidence intervals to scale uniformly across the different features, regardless of the SAGE value. But it's another for the largest confidence interval to shrink more slowly than it does with permutation sampling. I'm abandoning this now for SAGE, it does not appear to work.

I thought the derivations were cool, but it's all for nothing if this method is pointless. The only case I can come up with where it's not pointless is for SHAP, where the NeurIPS paper claims it's better than sampling. But that experiment is lacking a lot of details so it's hard to say for sure.
